Matching Papers and Reviewers at Large Conferences

Peer-reviewed conferences, the main publication venues in CS, rely critically on matching highly qualified reviewers for each paper. Because of the growing scale of these conferences, the tight timelines on which they operate, and a recent surge in explicitly dishonest behavior, there is now no alternative to performing this matching in an automated way. This paper studies a novel reviewer-paper matching approach that was recently deployed in the 35th AAAI Conference on Artificial Intelligence (AAAI 2021), and has since been adopted (wholly or partially) by other conferences including ICML 2022, AAAI 2022, and IJCAI 2022. This approach has three main elements: (1) collecting and processing input data to identify problematic matches and generate reviewer-paper scores; (2) formulating and solving an optimization problem to find good reviewer-paper matchings; and (3) a two-phase reviewing process that shifts reviewing resources away from papers likely to be rejected and towards papers closer to the decision boundary. This paper also describes an evaluation of these innovations based on an extensive post-hoc analysis on real data -- including a comparison with the matching algorithm used in AAAI's previous (2020) iteration -- and supplements this with additional numerical experimentation.

==> aaai21_paper_reviewer_matching (5)/MIP.tex <==

%, e.g., attempting to prevent malicious behaviour. 
%\citet{jecmen-etal-neurips2020} also tackles the issue of malicious behaviour via a randomized algorithm that relies on an externally provided list of suspicious (paper, reviewer) pairs. 
\newcommand{\constraintpar}[1]{\vspace{.6em}\noindent\textbf{#1}}

\subsection{MIP Problem Formulation}
\label{subsec: MIP_def}

% We now formally specify our mixed-integer program. Let there be
%  $N$ papers: $\papers = \{p_1, \ldots, p_{N}\}$, 
%  $M_{pc}$ Program Committee members (PCs): $\pcs = \{r_1, \ldots, r_{M_{pc}}\}$,
%  $M_{spc}$ Senior Program Committee members (SPCs): $\spcs = \{s_1, \ldots, s_{M_{spc}}\}$,
%  and $M_{ac}$ Area Chairs (ACs): $\acs = \{a_1, \ldots, a_{M_{ac}}\}$. We use the term \textit{reviewer} to refer to any of a PC, SPC or AC.% and let $M = M_r + M_s + M_a$ denote the total number of reviewers.
 
%\st{We now formally specify our mixed-integer program. Let there be $N$ papers, $M_\text{pc}$ Program Committee members (PCs), $M_\text{spc}$ Senior Program Committee members (SPCs), and $M_\text{ac}$ Area Chairs (ACs)  We denote the set of papers by $\papers$, the set of PCs by $\pcs$, the set of SPCs by $\spcs$, and the set of ACs by $\acs$. We also define the set of reviewers to be $\reviewers = \{ \pcs \cup \spcs \cup \acs \}$ and use the term \textit{reviewer} to refer to any of a PC, SPC or AC.}
%\nn{These M variables never get used. Why bother defining them}

We now formally specify our mixed-integer program. 
Let us denote the set of $N$ papers by $\papers$, the set of Program Committee members (PCs) by $\pcs$, the set of SPCs (Senior Program Committee members) by $\spcs$, and the set of Area Chairs (ACs) by $\acs$. We define the set of reviewers to be $\reviewers = \pcs \cup \spcs \cup \acs$ and use the term \textit{reviewer} to refer to any of a PC, SPC or AC.


 
 % and let $M = M_r + M_s + M_a$ denote the total number of reviewers.
 
 Our goal is to assign $\gamma_\text{pc}$ PCs, $\gamma_\text{spc}$ SPCs, and $\gamma_\text{ac}$ ACs to each paper $p_i$, for $1 \leq i \leq N$, such that the total reviewer--paper matching score is maximized subject to a set of constraints denoted by $\constraints$.
%Let $\assignmat$ be the $N_p \times M$ Boolean assignment matrix, where $\assignmatentry_{ij} = 1$ if $i^{th}$ paper is assigned to the $j^{th}$ reviewer, and $0$ otherwise.
%We use \textbf{bold case} for the variables to be assigned by the MIP, which includes the assignment matrix $\assignmat$ and various slack variables that are introduced as we relax certain hard constraints.
Our overall objective function not only includes the total matching score,
%$\matchingscore$, 
but also various penalties via the slack variables, due to violation of corresponding hard constraints.
%The overall assignment problem can be stated as:
%\begin{equation}
%    \max \ \obj \text{ \ subject to } \constraints
%\end{equation}
%\klb{You just said you bold variables. Does this assignment problem have no variables in it? I guess that makes it easy to solve :-)}
%\yn{$\obj$ is a function of both variables and constants, and is built incrementally, starting from  \cref{eq:matchscore}. 
%We are not using a bold face for functions, but only for variables. Should we instead use bold for functions as well?}
We initialize the overall objective function $\obj$ as the total matching score and then keep on adding terms to it as we relax the various constraints in the next section. 
We create binary variables $\assignmatentry_{ij}$ that denote whether paper $p_i$ is assigned to reviewer $r_j$.\footnote{In Phase 2, we set $\assignmatentry_{ij} = 1$ if $r_j$ was already assigned to $p_i$ in Phase 1 to ensure that the matching from Phase 2 is a superset of Phase 1 matching.
%\st{prevent a reviewer from being reassigned in Phase 2 to a paper that they were already assigned to in Phase 1.} 
The capacity limits on reviewers were increased accordingly.}
 We can write:
%Let $\scorematrix$ be a $N_p \times M$ score matrix with $\scorematrix[i,j]$ denoting the aggregate matching score between reviewer $j$ and paper $i$, as defined in Section~\ref{sec: scoring_function}.
%Then, the objective function $\obj$ is initialized by the total matching score as:
%Then, the matching score $\matchingscore$ is given by:
\begin{align}
\label{eq:matchscore}
\text{Initial Objective:~~}  \obj^\text{match} = \sum\limits_{i \in \papers, j \in \reviewers}
\scorematrixentry_{ij} \assignmatentry_{ij}.
\end{align}
Recall that $\scorematrixentry_{ij} \in [0,1]$ is the aggscore, the matching score between reviewer $r_j$ and paper $p_i$ as discussed in Section~\ref{sec: scoring_function}. Next, we formulate all the (soft) constraints in $\constraints$ as described earlier.

\subsection{Formulation of Constraints in $\constraints$}
\label{subsec: MIP_constraints}

\constraintpar{Constraint \ref{cons:coi}} (COI):
Let $\coimatentry_{ij} = 1$, if there exists a conflict of interest between reviewer $j$ and any of the authors of the paper $i$, and $0$ otherwise. 
%Refer to \cref{subsec: MIP_coi} for its computation.
%Obviously 
Reviewer $j$ cannot review paper $i$ if $\coimatentry_{ij} = 1$:
\begin{equation}
    \assignmatentry_{ij} = 0, \text{\  for each \ } i \in \papers, j \in \reviewers, \text{ \ such that \ } \coimatentry_{ij} = 1.
\end{equation}

%\klb{Use the same mechanism to prohibit a reviewer from being assigned in Phase 2 if they were already assigned in Phase 1?}


%\item \textit{Paper Capacity Constraints:}
\constraintpar{Constraint \ref{cons:numreviewers}} (Number of reviewers):
For each paper $p_i$, we need to ensure that it gets the desired number of reviewers:

\begin{comment}

\noindent \begin{equation}
    \label{eq:papercapacity}
    \sum\limits_{j \in \pcs} \assignmatentry_{ij} \leq \gamma_\text{pc} \ \ ; \ \ 
    \sum\limits_{j \in \spcs} \assignmatentry_{ij} \leq \gamma_\text{spc} \ \ ; \ \ 
    \sum\limits_{j \in \acs} \assignmatentry_{ij} \leq \gamma_\text{ac} .
\end{equation}

Usually these constraints will be tight because the scoring function is non-negative. However, it is possible to have a case in which conditional on the rest of the assignment, the only remaining matches do not contribute to the objective function. In such a case, the optimizer will not assign those papers their full capacity of reviewers since such assignments would be of poor quality.
%{\color{blue}Usually, these constraints will be tight because the scoring function is non-negative. However, suppose that the remaining matches do not contribute to the objective function, conditional on the rest of the assignment. In that case, the optimizer will not assign to those papers their full capacity of reviewers since such assignments would be of poor quality.}
We manually reviewed such cases.
%\yn{The above sentence was very long. I just tried to split it. Feel free to ignore if it is not good.}

\end{comment}
\noindent \begin{equation*}
    \label{eq:papercapacity}
    \sum\limits_{j \in \pcs} \assignmatentry_{ij} = \gamma_\text{pc} \ \ ; \ \ 
    \sum\limits_{j \in \spcs} \assignmatentry_{ij} = \gamma_\text{spc} \ \ ; \ \ 
    \sum\limits_{j \in \acs} \assignmatentry_{ij} = \gamma_\text{ac} 
\end{equation*}
With the equality constraints above, the MIP may become infeasible. Hence, we replace it with inequality constraints: 
\noindent \begin{equation}
    \label{eq:papercapacity}
    \sum\limits_{j \in \pcs} \assignmatentry_{ij} \leq \gamma_\text{pc} \ \ ; \ \ 
    \sum\limits_{j \in \spcs} \assignmatentry_{ij} \leq \gamma_\text{spc} \ \ ; \ \ 
    \sum\limits_{j \in \acs} \assignmatentry_{ij} \leq \gamma_\text{ac} 
\end{equation}
These constraints would be tight for a maximization problem where each match contributes positively to the objective. Note that it is possible to have a case in which conditional on the rest of the assignment, the only remaining matches do not positively contribute to the objective function. In such a case, the optimizer will not assign those papers their full capacity of reviewers since such assignments would be of poor quality.
We manually reviewed such cases.



\constraintpar{Constraint \ref{cons:reviewerload}} (Reviewer Load): The total number of papers assigned to a reviewer $j$ should not exceed their capacity $\capacity_j \in \mathbb{Z^+}$:
\begin{equation}
    \label{eq:reviewercapacity}
    \sum\limits_{i \in \papers} \assignmatentry_{ij} \leq \capacity_j, \forall j \in \pcs 
\end{equation}
\begin{equation*}
    \label{eq:reviewercapacity}
    \sum\limits_{i \in \papers} \assignmatentry_{ij} \leq \capacity_j, \forall j \in \spcs \cup \acs 
\end{equation*}
%\ycom{I seperated the equation for PCs and SPC/AC as we replace the hard constraints with soft ones only for SPCs and ACs}
%After the first round of assignments, we observed that the distribution of number of papers assigned to ACs and SPCs was very skewed with many ACs and SPCs not assigned even a single paper. 
Just ensuring the above upper bound may lead to an inequitable assignment of papers to reviewers, especially ACs and SPCs, many of whom may end up with no assignment at all. 
To resolve this, one option is to add a lower bound $\lowerlimitcapacity_j$ on the number of papers assigned to ACs and SPCs, as suggested by \citet{kobren&al19}:
\begin{equation*}
    \label{eq:reviewerlowerlimit}
    \sum\limits_{i \in \papers} \assignmatentry_{ij} \geq \lowerlimitcapacity_j, \forall j \in \spcs \cup \acs.
\end{equation*}
However, the lower bound constraint only ensures that no SPC or AC is unassigned, rather than preventing skewed matchings. %, with a reviewer $j$ assigned either $L[j]$ or $C[j]$ papers.
To promote an equitable distribution of papers amongst reviewers, we introduce $W$ intermediate capacity levels. For each $w \in \{1,2,\dots,W \}$, we define $\capacityentry_{jw}$
to be the intermediate capacity  for reviewer $j$ and set $\capacityentry_{j1}=\lowerlimitcapacity_j$ and
$\capacityentry_{jW} = \capacity_j$.
%We replace the hard constraints for ACs and SPCs with soft constraints to cause the system to prefer assigning $\capacityentry_{jw}$ papers to each reviewer $j$ as compared to assigning certain reviewers to their full capacity $\capacity_j$ while keeping others at their lower limit $\lowerlimitcapacity_j$. 
For ACs and SPCs, we replace the hard capacity constraints with a sequence of soft capacity constraints, one for each capacity level $w$. These constraints promote equitable distribution of papers as additional penalties are incurred each time an assignment crosses a new capacity level, making it very expensive to overload an individual.

To do so, we introduce new slack variables, $\capacityslack_{jw} \ge 0, \forall j \in \spcs \cup \acs, \forall w \in \{1 \ldots W\}$, each of which relax the capacity $\capacityentry_{jw}$ to  $\capacityslack_{jw} + \capacityentry_{jw}$, but penalize the objective by $\capacityslackpenalty_w(\text{type}_j)$ for each additional assignment above $\capacityentry_{jw}$, where $\text{type}_j$ denotes the reviewer category (SPC or AC). 
Then, for each $w \in \{1 \ldots W\}$:
\begin{align}
    \label{eq:reviewercapacityslack}
    \sum\limits_{i \in \papers} \assignmatentry_{ij} \leq & \  \capacityslack_{jw} + \capacityentry_{jw}, \ \  \forall j \in \spcs \cup \acs \text{ and } \forall w \in \{1 \ldots W\};  \\
    \label{eq:reviewercapacitypen}
    \obj^{\text{cap}} = &  \sum_{w \in W} \sum_{j \in \spcs \cup \acs} \capacityslackpenalty_w(\text{type}_j)\capacityslack_{jw}.
%    \obj   \pluseq& \  \obj_{rcap}[w]
\end{align}

%\nn{I understand the r is for reviewer, but I would leave it out and just call it cap. It looks like a typo}
% \yn{Should we write about our choice of W and Penalty matrix? We had it in the previous version. Pasting it below in blue}
% \cc{We added footnote in evaluation}
% {\color{blue}We kept $W=5$ with $\capacity[j,.]= [8,12,16,20,24] \forall j \in \spcs$ and $\capacity[j,.]= [20,30,40,50,60]$ for $j \in \acs$, with $\capacityslackpenalty[.,k]=-0.05, 1 \le w \le (W-1)$ and a very high penalty of $-0.5$ for $\capacityslackpenalty[.,W]$ for both SPCs and ACs, so that the system never assigns beyond $\capacity[j,W]=\capacity[j]$.}

\constraintpar{Constraint \ref{cons:seniority}} (Seniority):
%While assigning PCs, we want to encourage a spread of senior reviewers across papers such that each paper is likely to have senior input. 
We first assign $\text{seniority}_j \in \{0, 1, 2, 3\}$ to each reviewer $j$, such that $3$ is the senior-most category and $0$ is the junior-most category. In AAAI 2021, we chose to assign seniority levels as follows: Reviewers who had previously reviewed for at least 3 relevant conferences\footnote{Reviewers were asked: ``How many times have you been part of the Program Committee (as PC/SPC/AC, etc) of AAAI, IJCAI, NeurIPS, ACL, SIGIR, WWW, RSS, NAACL, KDD, IROS, ICRA, ICML, ICCV, EMNLP, EC, CVPR, AAMAS, HCOMP, HRI, ICAPS, ICDM, ICLR, ICWSM, IUI, KR, SAT, WSDM, UAI, AISTATS, COLT, CORL, CP, CPAIOR, ECAI, or ECML in the past?''} or had published 10 or more papers in relevant conferences were assigned seniority level $3$. Remaining reviewers having between 4 and 9 published papers were assigned seniority level $2$. Remaining reviewers having 2 to 4 papers or with experience reviewing at one or two previous conferences were assigned seniority level $1$. All other reviewers were assigned a seniority level of $0$.

We then reward each paper for maximizing its seniority level, up to some maximum reward. We introduce  slack  variables, $\seniorityslack_i\geq 0 ~ \forall i \in \papers$.
\begin{align}
    \label{eq:seniorityconstraints}
    \seniorityslack_i \leq& \sum\limits_{j \in \pcs} \text{seniority}_j \assignmatentry_{ij} , \forall i \in \papers \\
    \seniorityslack_i \leq& \text{~TargetSeniority}, \forall i \in \papers  \\
    \seniorityslack_i \geq& \text{~MinSeniority} , \forall i \in \papers \\
    \label{eq:senioritypenalty}
    \obj^{\text{sen}} =& \sum\limits_{i \in \papers} \seniorityreward \seniorityslack_i %\\
  %  \obj \  \pluseq& \ \obj_{sen}
\end{align}

Note that setting $\text{MinSeniority}$ greater than 0 can result in possible infeasibility (i.e., it may not be possible to assign a minimum level of seniority simultaneously to every paper). Setting $\text{MinSeniority}=0$ keeps the constraint soft. Papers are rewarded for seniority up to a maximum seniority level given by $\text{TargetSeniority}$. Setting this target allows us to express a preference for spreading seniority out over many papers rather than concentrating it on a few papers, as the objective only gets a bonus for the first $\text{TargetSeniority}$ units of seniority per paper. 

% \begin{align*}
% \small
%     \forall j &\in \pcs, \ \  j.seniority \\
%     =& 1 \text{\ if \ } (j.reviews \geq 3) or (j.papers  \geq 10) \\
%     =& 2 \text{\ elif \ } 4 \leq j.papers < 10 \\
%     =& 3 \text{\ elif \ } (1 \leq j.reviews < 3) or (2 \leq j.papers < 4) \\
%     =& 4 \text{\ otherwise}
% \end{align*}


\constraintpar{Constraint \ref{cons:coauthor} }(Coauthorship Distance):
This set of constraints penalizes the assignment of  pairs of reviewers who have ever coauthored a paper together to the same paper. This reduces the chances of papers' reviewers knowing each other, promoting review diversity.
To do so, for each pair of reviewers in $\coreviewerset = \{(j,j') | j < j', j,j' \in \pcs \cup \spcs\}$, we define a new variable $\coreview_{jj'} \ge 0$ such that it takes the value of $1$ if there exists a common paper assigned to both $j$ and $j'$, and $0$ otherwise. %\nn{The notation makes sense when we called these coreview constraints. Now that we call them coauthor constraints, a reader will get confused about why we are calling them cor}.
We exclude ACs from this set of constraints as they are few in number, highly trusted, and are not directly involved in discussions with the PCs.
%\hz{I think it would be enough to just say they are highly trusted}
The following constraints define $\coreview_{jj'}$: %, \forall (j,j') \in \coreviewerset$:
\begin{align}
    \coreview_{jj'} \ge& \ 0, \forall j,j' \in \coreviewerset; \\
    \coreview_{jj'} \ge& \ \assignmatentry_{ij} + \assignmatentry_{ij'} - 1, \ \ \forall i \in \papers \text{ and } \forall j,j' \in \coreviewerset.
\end{align}
Next, let $\coauthordist_{jj'}$ denote the edge distance between two reviewers $j$ and $j'$ in a coauthorship graph with reviewers as nodes. 
An edge exists between $j$ and $j'$ iff they have ever published a paper together (based on DBLP data, as described in Section~\ref{sec:COI}).
To discourage coauthors being reviewers of the same paper, we add a penalty that is bigger when coauthorship distance is small: 
\begin{align}
    \obj^{\text{co}} = & \sum\limits_{(j,j') \in \coreviewerset} p^{co}(\coauthordist_{jj'})\coreview_{jj'}.
  %  \obj \pluseq & \  \obj_{co}
\end{align}
$p^{co}(d)$ is the penalty coefficient, which depends on coauthorship edge distance $d$. We set $|p^{co}(1)| > | p^{co}(2) | > 0$ and $p^{co}(d) = 0, \forall d \ge 3$.

\constraintpar{Constraint \ref{cons:geo} }(Geographic Diversity):
For each paper $i$, let variable $\numregion_i$  count the number of distinct geographic regions of its assigned PCs and SPC. 
We inferred regions based on academic affiliations and email addresses provided by the reviewers. 
To encourage assignment of reviewers from different geographic regions, we add a reward proportional to $\numregion_i$ in the overall objective function so that $\numregion_i$ is maximized.
To count $\numregion_i$, we need to introduce auxiliary indicator variables, $\paperregion_{i\region} \leq 1$, that take the value of $1$ only if paper $i$ is assigned at least $1$ reviewer from region $\region \in \regions$.
%=\{\text{US,Asia,Australia,China,Europe}\}$.
Let $\reviewerregion_{j\region}$ indicate if reviewer $j$ belongs to region $\region$ or not.
%$\regions$ is the set of different regions to which reviewers belong. 
The following expressions define the overall regional constraints for each paper.
\begin{align}
    \label{eq:regionconstraints}
    \numregion_i \leq& \sum_{\region \in \regions} \paperregion_{i\region}, \ \forall i \in \papers \\
    \paperregion_{i\region} \leq& \sum\limits_{j \in \pcs \cup \spcs} \reviewerregion_{j\region} \assignmatentry_{ij}, \forall \region \in \regions \text{ and } \forall i \in \papers\\
    \paperregion_{i\region} \leq& \ 1,   \forall \region \in \regions \text{ and } \forall i \in \papers \\
    \label{eq:regionreward}
    \obj^{\text{reg}} =& \sum\limits_{i \in \papers} \regionreward \numregion_i 
%    \obj \  \pluseq& \ \obj_{reg}
\end{align}

\constraintpar{Constraint \ref{cons:cycle} }(No 2-Cycles):
These constraints aim to avoid scenarios where two reviewers both bid positively on each other's papers and are assigned these papers to review. Similar to Constraint \ref{cons:coauthor} (Coauthorship Distance) and \ref{cons:geo} (Geographic Diversity), we exclude ACs from this constraint for similar reasons.
We first identify all such bidding cycles, where reviewer $j$ bids positively on paper $i$ authored by reviewer $j'$ and $j'$ bids positively on paper $i'$ authored by reviewer $j$, with $j,j' \in \pcs \cup \spcs$.
Denote such a bidding cycle by a 4-tuple $(j,j',i,i')$, and the set of all such cycles as $\cycles$.
We then aim to avoid any of the assignments in the bidding cycle $(j,j',i,i')$.
We introduce slack variables, $\cyclevars_{jj'ii'} \geq 0$, for each bidding cycle, and add a penalty $\cyclepen$ in Equation~\eqref{eq:cyclepenalty} for every assignment that belongs to a bidding cycle.\footnote{In the conference and this paper's experiments, we used an alternate formulation of the constraint which only penalized bidding cycles that led to assignment cycles. In this formulation, slack variables $\cyclevars_{jj'}$ were created for each pair of reviewers $(j,j')$ involved in a bidding cycle, and the constraint was enforced with $\assignmatentry_{ij} + \assignmatentry_{i'j'} \leq (1 + \cyclevars_{jj'})$. We present the above formulation instead because, on reflection, we recommend penalizing both halves of a cycle separately.}
\begin{align}
    \label{eq:cycleconstraints}
    \assignmatentry_{ij} \leq& \  \cyclevars_{jj'ii'} , \forall j,j',i,i' \in \cycles \\
    \label{eq:cyclepenalty}
    \obj^{\text{cy}} =&  \sum\limits_{j,j',i,i' \in \cycles} \cyclepen \cyclevars_{jj'ii'} 
 %   \obj \  \pluseq& \ \obj^{cy}
\end{align}


%  First, because the relaxation doesn't actually do this---it penalizes each person in the cycle separately, whether or not the second person gets assigned. This is not a relaxation of the hard constraint stated, it's a relaxation of a strengthening of that constraint (basically, it relaxes treating membership in a 2-cycle as a COI). Second, because the soft constraint makes \textit{more} sense than the hard constraint. If a cycle is fishy, why is it OK to have half of it? Rewrite to eliminate the hard constraint or to specify it as a COI. This will make the whole thing easier to explain and also more correct.}

% \yn{Good point: the constraints above are indeed implying that its okay to have one assignment from the bidding cycle but not two. We pay a penalty only when \textit{both} are assigned. 
% I don't see how is it penalizing each person in the cycle separately, irrespective of the second person getting assigned or not: the slack variable $\cyclevars[j,j']$ gets a value of 1 only when \textit{both} $\assignmatentry_{ij}$ and $\assignmat[i',j']$ are 1. 
% Am I missing something?}

Finally, our overall assignment problem can be stated as:
\begin{align*}
    &\text{max} \ \obj = \obj^\text{match} + \obj^{\text{cap}}+ \obj^{\text{sen}}+ \obj^{\text{co}} + \obj^{\text{reg}} + \obj^{\text{cy}} \\
    &\text{subject to } \constraints.
\end{align*}



==> aaai21_paper_reviewer_matching (5)/MIP_scalability_evals.tex <==
We now turn to an evaluation of our matching algorithm (described in \Cref{sec: MIP}), including a comparison to the matching algorithm used at AAAI 2020, the previous year's conference. 
For our experiments, we created a full conference dataset containing all submitted AAAI 2021 papers and reviewers analyzed above. We augmented the dataset to include all additional reviewers who were not ultimately assigned any reviews at AAAI 2021, bringing the total number of reviewers up to 8,964. Except where otherwise noted, we evaluated our algorithm in terms of the single-phase matching problem, as this allows us to focus on matching quality and facilitates comparison with prior work. In the same spirit, we required each paper to be assigned four reviews ($\gamma_\text{pc}=4$) and set a limit of five reviews per reviewer ($\capacity_j = 5$). We ran row generation (as described in \Cref{subsubsec:rowgen}) for 10 iterations. We ran all of our experiments on a 16-core machine with Intel Silver 4216 Cascade Lake 2.1GHz processors and 96 GB RAM. For MIP solving, we used CPLEX version 12.9.0.0 with default parameters. 

We note a subtlety that arises when comparing different assignments. Recall that we used an inequality instead of a hard constraint on the number of matches each paper receives, allowing the MIP to assign fewer than $\gamma_\text{pc}$ reviewers to a paper. This can occur for papers for which there are no qualified reviewers or only very poor matches conditional on the rest of the assignment. A consequence is that we can find ourselves needing to make comparisons across assignments in which different numbers of reviewer--paper matches exist. In these cases, we padded all matchings with reviewer--paper matches that contributed nothing to the objective function, as though we had matched the paper to a reviewer having an aggscore of 0 who imposed neither rewards or penalties via soft constraints. Such zero-contribution matches accounted for at most 1\% of the total reviews in any of our matchings reported below. While in reality we addressed all such cases at AAAI 2021 manually, we note that many AAAI 2021 reviewers were ultimately assigned zero papers, meaning that a large pool of available and unused reviewers did exist.

\subsubsection{How did our algorithm compare to the algorithm used in the previous iteration of the conference?}

We compared our matching algorithm to the method used in the conference's previous iteration (AAAI 2020), a flow-based matching algorithm. Rather than simple capacity constraints, each paper and reviewer had a number of weighted \emph{slots} that linearly scaled the contribution of each assignment to prioritize each paper getting some good reviewers and each reviewer getting some good papers. Based on advice from the previous Program Chairs, we set the paper slot weights to be 8/4/1/1 and reviewer slot weights to be 8/2/1/1/1. Their reviewer--paper scoring function differed from ours in two main ways: (1) it did not use ACL scores, and (2) bids scaled scores multiplicatively rather than exponentially. Beyond the scoring function, their matching algorithm did not attempt to satisfy any soft constraints.

% Their code snippet: assignment_scores = (beta*subject_scores+(1-beta)*tpms_scores)*(gamma**(bids+sugg))
Nevertheless, we investigated how effective last year's approach was at limiting soft constraint violations despite not optimizing for them (i.e., we tested how frequently these violations occurred organically at the optimum of a simpler matching problem). We ran both algorithms and evaluated the number of soft constraint violations compared to our approach. For reference, we also performed a similar experiment that compared our AAAI 2021 algorithm to a version of the same algorithm that omitted all soft constraints. We summarize the results in \Cref{tab:constraint_improvement_over_2020}, reporting the percent reduction in the number of:
(a) papers without a senior reviewer (Constraint \ref{cons:seniority});
(b) coauthor violations (Constraint \ref{cons:coauthor});
(c) papers with reviewers from the same region (Constraint \ref{cons:geo}); and
(d) cycle violations (Constraint \ref{cons:cycle}).
We observed that AAAI 2020's approach led to substantially more violations of three of the four soft constraints. Most notably, our algorithm assigned to the same paper 76.8\% fewer pairs (118 compared to 509) of reviewers who were previous coauthors . Conversely, our approach led to a 90\% \emph{increase} in the number of violations of our no-2-cycles constraint, prohibiting pairs of reviewers who bid positively on each other's submissions from being assigned to each other's papers. However, such matchings were quite rare overall (22 for AAAI 2020 and 42 for our approach out of 26,916 reviewer--paper matchings in total).
%6,729 papers receiving 4 reviews each). 
We believe that the AAAI 2020 method led to fewer 2-cycles because their scoring function weighs positive bids less heavily than ours does and therefore is less likely to match reviewers to papers where a reviewer bid positively.
When using our scoring function, we were able to reduce 2-cycle violations by 84\% using our soft constraint over the baseline version with no soft constraints.

Our algorithm had approximately the same memory footprint as the flow-based approach (96 GB vs 95 GB) despite the additional soft constraints that our method considered: the flow-based method creates an edge for every reviewer--paper pair whereas we only created variables for a subset of qualified reviewers. In terms of runtime, running our algorithm with 10 iterations of row generation required 52.0 wall-clock hours compared to 0.8 needed for the AAAI 2020 approach. Note that our approach is anytime: it can terminate after any number of iterations of row generation. One iteration of our algorithm took 0.9 wall-clock hours and five iterations took 7.3 wall-clock hours.
%The much larger wall-clock of our approach is expected since our method solves 10 iterations of MIPs whereas they can solve their matching optimally in polynomial time.  
We were willing to devote a few days to computation, so we find these numbers reasonable. Nevertheless, in what follows we identify some ways to reduce runtimes without sacrificing much in performance (e.g., $5\times$ speedup via decomposing the matching into two stages; $1.7\times$ speedup via reducing $k$ to further sparsify the constraint matrix).
%3096 after 1 iter of row gen, 26307.65873646736 after 5 iter
\begin{table*}
\begin{center}
\small
\begin{tabular}{ l| r r}
\toprule
 \textbf{Soft constraint} & \textbf{Baseline (no soft constraints)} & \textbf{AAAI 2020} \\
 \midrule
  \textbf{Constraint \ref{cons:seniority}} (Seniority) & 56.1 & 9.5\\
  \textbf{Constraint \ref{cons:coauthor}} (Coauthorship Distance) & 88.1 & 76.8\\
%   Papers w/ near coauthor reviewers ($Pen_{co}(1)$) & 54.8\\
  \textbf{Constraint \ref{cons:geo}} (Geographic Diversity) & 24.1 & 23.3\\
  \textbf{Constraint \ref{cons:cycle}} (No 2-Cycles) & 84.6 & -90.9\\
  %' Match Quality & 40.9 & ?\\
  \bottomrule
\end{tabular}
\caption{Percent reduction of soft constraint violations using our approach relative to (1) our approach without soft constraints and (2) last year's matching algorithm for a simulation of a single-phase version of AAAI 2021.}
\label{tab:constraint_improvement_over_2020}
\end{center}
\end{table*}
%\yn{Would it make sense to report total number of violations using our method in \cref{tab:constraint_improvement_over_2020}, in addition to the percentage reductions?}
%\cc{We decided absolute numbers were difficult to interpret unless small number}
% \begin{comment}
% \begin{table}
% \begin{center}
% \small
% \begin{tabular}{ l{1cm}| r r}
% \toprule
%  Soft constraint & Baseline (no soft constraints) & AAAI 2020 \\
%  \midrule
%   Papers w/ coauthor reviewers ($Pen_{co}(0)$) & 88.1 & 76.8\\
% %   Papers w/ near coauthor reviewers ($Pen_{co}(1)$) & 54.8\\
%   2-cycles & 84.6 & -90.9\\
%   Papers w/ reviewers from same region & 24.1 & 23.3\\
%   Papers w/ no senior reviewer & 56.1 & 9.5\\
%   %' Match Quality & 40.9 & ?\\
%   \bottomrule
% \end{tabular}
% \caption{Percent reduction of soft constraint violations using our approach relative to (1) our approach without soft constraints and (2) last year's matching algorithm for a simulation of a single-phase version of AAAI 2021.}
% \label{tab:constraint_improvement_over_2020}
% \end{center}
% \end{table}
% \end{comment}
\subsubsection{What did introducing soft constraints cost us in matching aggscore?}\label{subsec:softeval}
%We define in our objective function the tradeoffs between agg score and soft constraint violations but how much agg score reduces with soft constraints is a property of the dataset. 
Table \ref{tab:improvement_over_2020} shows that for the most part, with our specific settings of the soft constraint parameters, we were able to have our cake and eat it too. With all of our soft constraints turned on, we only lost 2.04\% mean aggscore. With each soft constraint turned on individually, the Coauthorship Distance and Geographic Diversity constraints reduced mean aggscore the most (1.17\% and 0.85\% respectively) while the Seniority and No 2-Cycles constraints reduced mean aggscore the least (0.05\% and 0.01\% respectively). 
The sum of the aggscore reductions across matchings where each soft constraint was turned on individually was 2.08\% (sum of first four rows in Table \ref{tab:improvement_over_2020}), very similar to the 2.04\% reduction in mean aggscore when all constraints were turned on simultaneously. This suggests that there was very little complementarity across different constraints (e.g., when we reduced Coauthorship Distance violations, we rarely also increased Geographic Diversity as a side effect).

\begin{table*}
\begin{center}
\small
\begin{tabular}{ l r}
\toprule
 \textbf{Soft constraint} & \textbf{\% Aggscore reduction} \\
 \midrule
 \textbf{Constraint \ref{cons:seniority}} (Seniority) & 0.05\\
 \textbf{Constraint \ref{cons:coauthor}} (Coauthorship Distance) & 1.17 \\
 \textbf{Constraint \ref{cons:geo}} (Geographic Diversity) & 0.85\\
 \textbf{Constraint \ref{cons:cycle}} (No 2-Cycles) & 0.01\\
 \midrule
 All constraints & 2.04 \\
  \bottomrule
\end{tabular}
\caption{Percent reduction in aggscore when each soft constraint was turned on individually relative to a base MIP having no soft constraints. The final row displays the reduction when all soft constraints were present.}
\label{tab:improvement_over_2020}
\end{center}
\end{table*}

\begin{comment}
\begin{table*}
\begin{center}
\small
\begin{tabular}{ l r}
\toprule
 \textbf{Soft constraint} & \textbf{\% Aggscore reduction} \\
 \midrule
 Papers w/ coauthor reviewers ($Pen_{co}(0)$) & 1.17 \\
 Regions per paper & 0.85\\
 Papers with no senior reviewer & 0.05\\
 Cycle violations & 0.01\\
 \midrule
 All constraints & 2.04 \\
  \bottomrule
\end{tabular}
\caption{Percent reduction in aggscore when each soft constraint was turned on individually relative to a base MIP having no soft constraints. The final row displays the reduction when all soft constraints were present.}
\label{tab:improvement_over_2020}
\end{center}
\end{table*}
\end{comment}
\subsubsection{How well did the row generation of coauthorship distance constraints perform?}
\label{subsec:roweval}
Ideally we would evaluate the performance of the row generation of coauthorship distance constraints by comparing performance after each number of iterations to the performance of the optimal approach that held all rows of the constraint matrix in memory. Unfortunately, we were unable to compute the optimal objective value (OPT) for our dataset: this is why we needed row generation in the first place! Nevertheless, we can compare to an upper bound on OPT. 
% {\color{blue}In each iteration, we maximize the objective function without the soft penalty for coauthorship constraint violations and forbid violating assignments from the previous iterations.
% Since each additional coauthorship constraint in the successive iterations can only penalize the objective function being maximized (\ie, objective function without soft penalty for coauthorship constraints), it can only weakly decrease as these constraints are added. Therefore, the objective value (without coauthorship penalty) that we obtain after the last iteration of row generation (\cref{alg:itersolve}) is an upper bound on OPT. 
% After 10 iterations, we closed the gap between the first iteration and the upper bound on OPT by 77.5\%.
% Notice that the gap is computed between the upper bound on OPT and the objective value \emph{with} the coauthorship penalty and that the gap may or may not decrease monotonically with each iteration. 
% }
Since each additional coauthorship constraint can only penalize the objective function, the optimal value of the objective function (without coauthorship penalty from ungenerated constraints) can only weakly decrease as these soft constraints are added. Therefore, the objective value we observe after the last iteration of row generation is an upper bound on OPT.
%After 10 iterations, we closed this gap by 77.5\% between the initial solution before row generation and the upper bound on OPT.
After 10 iterations, we closed the gap between the initial solution before row generation (obtained with $\coreviewerset_0$ in \Cref{alg:itersolve}) and the upper bound on OPT by 77.5\%.

%\todo{Yatin: Please review the text above. I hope it adds more clarity}

\subsubsection{How did the choice of our column generation parameter $k$ impact the objective?}
Recall that to reduce the size of our MIP, we created variables only for the most-promising paper--reviewer pairs: for each reviewer, we sampled the $k$ best-scoring papers, and for every paper, we sampled the $k$ best-scoring reviewers. We then filtered out any paper--reviewer pairs scoring below a threshold, keeping only qualified reviewers. We set $k=50$ when creating the match for AAAI 2021. %Figure \ref{fig:qualified} shows that the median paper has 1446 qualified reviewers; when conditioning on reviewers that placed positive bids, the median paper has 43 qualified reviewers. 
\Cref{fig:qualified} shows that after this filtering, the median paper had $\approx$1,500 qualified reviewers. 
Expanding to include variables for all possible qualified assignments (unbounded $k$) would have required much more memory than was available via our computing resources.

We investigated the impact of $k$ on the quality of the resulting matching. Running our algorithm with a much smaller $k$ value ($k=10$), we observed only a 1.8\% loss in the objective but a 1.7 times speedup in performing 10 iterations of row generation, as compared to $k=50$. Increasing $k$ to $100$ had a negligible impact on the objective (0.04\%). We consider it unlikely that significant additional gains would be achieved by even further increases to $k$. 

%While column generation was not strictly required for AAAI 2021 (a fact only obvious in hindsight; many design decisions were in flux leading up to the matching), it provides a way to scale our algorithm to settings where it would not be possible to consider all possible qualified assignments in memory.

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\textwidth]{figures/aggscore_v_rank}
%     \caption{\nn{Relabel figure with mean aggscore. Confirm this is on the right dataset}. Mean aggscore of each paper's $k$th best reviewer. The red line represents the 50th ranked reviewer. Quality drops sharply, so $k=50$ is a sufficiently high parameter.\label{fig:aggscore_v_rank}}
% \end{figure}
\begin{figure*}[t]
\centering
  \includegraphics[width=0.45\textwidth]{figures/qualified}\hspace{.09\textwidth}
  \includegraphics[width=0.45\textwidth]{figures/qualified_that_bid}
  \caption{ECDF of the number of ``qualified'' reviewers for each paper (i.e., reviewers with $\scorematrixentry_{ij} \geq 0.15$), considering both all reviewers (Left) and only reviewers who also made a positive bid for the paper (Right). The median paper had 1446 qualified reviewers and 43 qualified reviewers who also placed a positive bid.\label{fig:qualified}}
\end{figure*}
% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.75\textwidth]{figures/bidscdf}
%   \caption{\nn{Reformat with larger text} ECDF of the number of positive bids (at least \emph{in a pinch}) for each paper.\label{fig:bidscdf}}
% \end{figure}

\subsubsection{What were the tradeoffs between objective value and computational savings with multiple phases?}

In a two-phase conference, about half of the total reviews are assigned in each phase, so the Phase 1 and Phase 2 MIPs have half as many free variables as the MIP for a corresponding single-phase conference.  We should expect solving the two smaller problems to be much faster than solving the larger one, since the running time of MIP solvers tends to scale superlinearly with problem size. However, of course, the solution obtained by solving two phases optimally in succession will yield weakly lower objective value than the optimal solution to the single-phase problem. For example, imagine that each stage assigns two reviews per paper and that for some paper, there are only four qualified reviewers. The two-phase algorithm will not consider that it may need to save two qualified reviewers for the second phase, and may assign these highly specialized reviewers elsewhere, consuming their capacity. We thus empirically evaluated loss in objective value due to running a two-phase version of our conference. In these experiments, we assigned two reviewers per paper in Phase 1, fixed those assignments, and then assigned two more reviewers per paper in Phase 2. We found that the resulting matching had objective value only 0.02\% lower, as compared to the single-phase conference. On the other hand, decomposing the problem in this way led to a $5\times$ speedup.

It occurred to us that this approach of incrementally building up a MIP solution reviewer by reviewer did not require that the conference actually did perform two-phase reviewing. For example, a single-phase conference could use this same two-phase strategy simply to speedup MIP solving, which could make a significant computational difference for conferences significantly larger than AAAI 2021. To investigate this idea, we evaluated a four-phase approach that assigned one reviewer per paper, fixed those assignments, and repeated four times until each paper had four reviewers. As before, we observed very encouraging results: the objective value decreased by only 0.33\% relative to a single-phase conference, whereas MIP solving was accelerated by 28$\times$ (see \Cref{tab:multi-phase})!

\begin{table}
\begin{center}
\small
\begin{tabular}{ l r r}
\toprule
 \textbf{Number of phases} & \textbf{Objective reduction} & \textbf{Speed up}\\
 \midrule
2 & 0.02\%  & 5.4$\times$ \\
4 & 0.33\%  & 28.1$\times$ \\
  \bottomrule
\end{tabular}
\caption{Sacrifice in objective function vs. computational savings of multi-phase conferences relative to single-phase conference.}
\label{tab:multi-phase}
\end{center}
\end{table}

% Single stage experiment

% Running time: 31549.72 CPU seconds
% Objective: 31701.00

% Two-stage experiment (what we did in conference)

% Running time (phase 1): 2643.01 CPU seconds
% Running time (phase 2): 459.14 CPU seconds
% Total running time (phase 1): 3102.14 CPU seconds
% Objective: 31549.72

% 202.7 times faster, 0.48\% loss in objective.

% Four-stage experiment (what we did in conference)

% Running time (phase 1):  102.60 CPU seconds
% Running time (phase 2):  255.30 CPU seconds
% Running time (phase 3):  69.15 CPU seconds
% Running time (phase 4):  278.03 CPU seconds
% Total running time (phase 1):  705.09 CPU seconds
% Objective: 

%  times faster, \% loss in objective.




\subsubsection{How did our algorithm scale?}

To understand how our algorithm's performance depended on the size of the conference, we generated 77 synthetic conferences of different sizes by subsampling papers and reviewers (without replacement) from our dataset. In an attempt to maximize the realism of the structure of our simulated conferences, we constructed them based on related keywords. At AAAI 2021, keywords were divided into top-level categories (e.g., Machine Learning) and bottom-level categories (e.g., Learning Theory); papers and reviewers could select one top-level and multiple bottom-level keywords.

Our generator works as follows. We begin with an initial bottom-level keyword and then initialize our conference to contain all papers associated with that keyword and a set of reviewers associated with the corresponding top-level keyword proportional to the fraction of papers belonging to the bottom-level keyword within that top-level area. We store a set of keywords associated with our conference as the generator runs. In each iteration, we add to our set of keywords the keyword belonging to most papers in our current set of papers that is not yet part of our tracked set of keywords. Papers corresponding to this keyword and additional reviewers are then added accordingly. 
Every time the number of papers grew by a constant factor, we created a new synthetic conference containing the current set of papers and reviewers and added it to our set of samples.
For diversity, we ran our generator on three trajectories, each seeded with a different keyword: one from game theory, one from computer vision, and one from constraint satisfaction, because each of these areas involves a substantially  distinct set of reviewers and authors and each has its own dedicated conferences. We also included the full AAAI 2021  dataset as our final datapoint, giving us a total of 78 simulated conferences.
%\klb{This could be a bit more precise, but maybe it's ok.}
  %GameTheoryandEconomicParadigms:Equilibrium, ComputerVision:ObjectDetection and Categorization, and ConstraintSatisfactionandOptimization:ConstraintSatisfaction. We ended up with 78 subconferences.


\begin{figure*}[t]
\centering
    \includegraphics[width=.6\textwidth]{figures/scaling_row_gen}
    \caption{Running time vs. conference size (number of papers); points represent (conference, iteration) pairs.\label{fig:scale}}
\end{figure*}

%\paragraph{How did row generation approach scale?}
%using paragraph was resulting in an additional fullstop after question mark.
% \noindent \emph{How did row generation approach scale?}
We then turned to studying how our row generation approach scaled. Figure~\ref{fig:scale} shows cumulative wall-clock time for each (conference, iteration) point. Points are coloured by iteration. For conferences with fewer than 1,000 papers, we could always complete 10 iterations in less than an hour. Interestingly, the smallest conferences were harder to optimize than medium-sized conferences. We speculate that this occurred because some soft constraints (e.g., coauthor / cycle constraints) were harder to satisfy when the set of papers and reviewers were more densely connected. Running time appeared to scale exponentially as the number of papers grew beyond 1,000, with the biggest size taking a few hours per iteration.

\begin{figure*}[t]
\centering
  \includegraphics[width=.6\textwidth]{figures/gap_closed_row_gen_by_iter}
  \caption{ECDF of \% of gap closed (relative to our upper bound) between the first and $k^{th}$ iteration of row generation.\label{fig:optgap}}
\end{figure*}

\subsubsection{How did our results on optimality and aggscore reduction translate to our generated conferences?}

\Cref{fig:optgap} shows ECDFs of how much of the gap we closed between the initial solution before row generation and the upper bound on OPT described earlier in \Cref{subsec:roweval}. After just one iteration of row generation, we closed at least 25\% of the gap for 80\% of the generated conferences.  After 10 iterations, we closed 75\% of the gap for over 90\% of conferences. The trend in which these ECDFs become closer and closer together after successive iterations led us to believe that we were approaching optimality, and that much of the remaining 
%25\% of the 
gap after 10 iterations was due to looseness in our upper bound on OPT.
%\yn{If upper bound becomes tight, wouldn't it further increase the gap from 25\%? yes!}
\begin{figure*}[t]
\centering
  \includegraphics[width=.6\textwidth]{figures/agg_score_reduction.pdf}
  \caption{ECDF of the fractional reduction in mean aggscore upon adding soft constraints.}\label{fig:agg_score_reduction}
\end{figure*}


Similar to the results previously reported about our full conference in \Cref{subsec:softeval}, we observed that introducing soft constraints led to only small reductions in aggscore across our 77 variable-sized conferences. For 60\% of these conferences, we lost less than 2\% in aggscore; at worst, we lost 5\%.  
\Cref{fig:agg_score_reduction} shows an ECDF of the reduction in aggscore across all the generated conferences.










==> aaai21_paper_reviewer_matching (5)/MIP_solving.tex <==
% \subsection{Scaling}

Given our formulation, instantiating a variable $\assignmatentry_{ij}$ for each possible (reviewer $j$, paper $i$) combination, along with all of the associated slack variables and constraints, would lead to a MIP too large to store in memory, let alone to solve. We therefore applied column (variable) generation, only creating variables for a subset of all possible assignments and employed row (constraint) generation. %\klb{Shouldn't this be column (variable) generation? Or do you mean that additionally you performed row generation for one of the constraints (as I do realize you did)? But you must have also done column generation in the case where the MIP was infeasible with the initially generated variables. BTW, if you disagree with me here, take out my reference to column generation in the introduction. But I do think that generating only some of the variables is in some sense column generation, even if you didn't iterate. Perhaps we should discuss.}

\subsubsection{Generation of Assignment Variables} We only created $x_{ij}$
%\st{entries in $\assignmatentry_{ij}$ for}\todo{Yatin: In the new notation, $x$ is no longer a matrix. So entries in %$x_ij$ doesn't sound right.
%}
variables that were likely to be relevant (thereby restricting the space of possible assignments; implicitly, non-generated variables are set to 0). There was little point in considering variables that correspond to $(i,j)$ pairs with low matching scores, as these would represent poor matches.  In rare cases, this may result in papers receiving fewer than the desired number of reviews. When the MIP is infeasible in this way, one can iterate (perform column generation) by generating more matching variables for the corresponding papers. However, at AAAI we assigned matches to such papers manually, as the algorithm is unlikely to do much better than a random assignment when given only low-scoring alternatives. %We recommend that such papers be assigned matches manually, as the algorithm is unlikely to do much better than a random assignment when given only low-scoring alternatives.
%\yn{The two lines above are very similar. Lets have only one of them?}
We did not create variables for any reviewer--paper pair $(i,j)$ with $\scorematrixentry_{ij} < 0.15$.\footnote{We note that this suggests a refinement to the bidding procedure: it is only necessary to show reviewers papers for which a sufficiently positive bid could bring their score above the threshold. This could result in large time savings for reviewers in the bidding phase, as it can be hard to sift through an entire conference worth of papers.} 

We created variables as follows: for each paper, we created a variable for the $k$ highest scoring PC, SPC, and AC reviewers. Similarly, for each PC/SPC/AC member, we created a variable (if it did not exist already) for their highest scoring $k/5k/10k$ papers. 
%\klb{As discussed above, I'd define the method in terms of column generation and then say we didn't iterate, in part for the reasons you give here and in part because of the argument about low scoring matches being unreliable.} 
$k$ can be iteratively expanded as time allows (perhaps in a targeted way, such as increasing $k$ for underutilized reviewers) until the dense matrix is recovered. However, our MIP was computationally feasible at high enough $k$ that further increases to $k$ offered only negligible improvements, so we did not iteratively perform column generation. 

\subsubsection{Generation of Coauthor Constraints}\label{subsubsec:rowgen}
%CC: Use \Gamma in text
% Use V_{i}
Even given our reduced $k$, there were too many coauthor constraints to include (the number scales with the product of the number of $\assignmatentry_{ij}$ variables and the number of reviewers).
Instead, we started solving the problem with no coauthor constraints. After reaching an initial solution, we identified violated coauthor constraints and added them explicitly to the MIP. We repeated this process until we were satisfied with the number of violated constraints; in practice the number of violations plateaued after eight iterations. %Additionally, after each iteration we added an additional factor of $k$ variables for any unused reviewer.\hz{why is this a good idea?} 
Pseudocode %for our generation algorithm 
is given as Algorithm~\ref{alg:itersolve}.

\begin{algorithm}[H]
\begin{algorithmic}[1]
\small
\caption{Assignment Variable Sparsification and Constraint Generation}
\label{alg:itersolve}
\STATE Let $\coreviewerset_{\text{master}}$ contain all coauthor constraints
%\STATE Let $k$ be an initially chosen matrix dimension
%\STATE Compute a sparse matrix $\assignmat_k$ by sampling a constant multiple of the top $k$ papers for every reviewer and top $k$ reviewers for every paper
\STATE Let $\assignmat_k$ be the set of $x_{ij}$ variables obtained by sampling a constant multiple of the top $k$ papers for every reviewer and top $k$ reviewers for every paper

\STATE $i \gets 0$
\STATE $\coreviewerset_{i} \gets \{\}$ \COMMENT{Store of violated coauthor constraints up to iteration $i$, initially empty}
\WHILE{True}
    \STATE Solve the MIP defined by $\assignmat_{k}$ and $\coreviewerset_i$. Store the solution in $\assignmat^*$
    \STATE Identify all new coauthor violations $\coreviewerset_{\text{new}}$ in $\assignmat^*$ using $\coreviewerset_{\text{master}}$
    \IF{$V_{\text{new}}$ is empty or time has run out}
        \STATE Return $\assignmat^*$
    \ENDIF
    \STATE $\coreviewerset_{i+1} \gets \coreviewerset_{i} \cup \coreviewerset_{\text{new}}$
    \STATE $i \gets i+1$
   % \STATE For any unused reviewer in $\assignmat^*$, add variables for an additional $k$ papers to $\assignmat_k$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

Lastly, to reduce computation time, we did not attempt to find an optimal solution to the MIP.
Instead, we set an absolute MIP-gap tolerance of $20$. Since aggscore is on a scale between $0$ and $1$ and we make on the order of tens of thousands of assignments, being suboptimal by at most $20$ objective function units is relatively benign. The result was that we found a very nearly optimal solution much more quickly.


%\noindent The MIP as formulated above is too large to practically write out and feed into a commercial solver.
%In the next sub-section, we describe the tricks and methods used to solve the MIP efficiently.
%In \cref{sec:MIP_inputs}, we describe the technical details of the most crucial inputs to the MIP, \ie, the scoring matrix, $\scorematrix$, and the COI matrix, $\coimat$.




==> aaai21_paper_reviewer_matching (5)/abstract.tex <==
% %  We begin with automated conflict identification and bid preprocessing algorithms that reduce opportunities for manipulation. These feed into a scoring function that combines information across many sources to assess the quality of (paper, reviewer) pairs and is robust to missing data. We optimize these scores via a scalable Mixed-Integer Programming (MIP) formulation that also rewards geographic diversity among co-reviewers, light reviewer workloads, and an even spread of senior reviewers across papers. Our MIP further penalizes assignments with the potential to facilitate malicious behavior: close colleagues reviewing the same paper, and authors reviewing each other's papers. This paper also introduces a novel two-phase reviewing scheme which shifts reviewing resources away from papers that almost certainly will be rejected and towards borderline papers.

% Peer-reviewed conferences, the main publication venues in CS, rely critically on matching highly qualified reviewers for each paper. Because of the growing scale of these conferences, the tight timelines on which they operate, and a recent surge in explicitly dishonest behavior, there is now no alternative to performing this matching in an automated way. 
% %For example, x papers were submitted to AAAI in 2021, as compared to only y in AAAI-2015.
% %With the unprecedented scale of the conferences, it is not possible to manually match reviewers to the papers and hence to ensure fair and equitable assignment of reviewers to the papers, creating an unbiased automated matching process becomes crucial.
% %
% %This paper proposes a suite of methods for matching papers with reviewers that maintain high quality standards, ensure fairness, and reduce the effectiveness of various forms of malicious behavior. 
% %
% %Ensuring that our reviewing mechanisms continue to function well is critical to the continued health of our field.   
% %In the recent past, many authors have complained on social media about poor quality of reviews, reviews going unchecked even by Senior Program Committee members and Area Chairs, demonstrating either a dearth of good reviewers, or issues with the existing reviewer--paper matching systems.  %%%%
% %Approaches that work for conferences with hundreds of submissions break down when both papers and reviewers number in the thousands. %Another challenge is a recent surge in explicitly dishonest behavior such as collusion rings, where authors collude to bid on each others' papers with the goal of submitting fraudulent reviews. 
% This paper studies a novel reviewer--paper matching approach that was recently deployed in the 35th AAAI Conference on Artificial Intelligence (AAAI 2021), and has since been adopted by other conferences including AAAI 2022 and ICML 2022. This approach has three main elements: (1) collecting and processing input data to identify problematic matches and generate reviewer--paper scores; (2) formulating and solving an optimization problem to find good reviewer--paper matchings; and (3) a two-phase reviewing process that shifted reviewing resources away from papers likely to be rejected and towards papers closer to the decision boundary.
% % We aim to convince the reader that both of these problems can be mitigated by the application of AI techniques, assessing the usefulness of our methods on real data from the 35th AAAI Conference in Artificial Intelligence (AAAI 2021).
% This paper also describes an evaluation of these innovations based on an extensive post-hoc analysis on real data---including a comparison with the matching algorithm used in AAAI's previous (2020) iteration---and supplements this with additional numerical experimentation.\footnote{Writing this paper and conducting the experimental analysis described herein took almost a full year beyond the conclusion of AAAI 2021. Nevertheless, this paper is grounded in our experiences as Program Chairs (Mausam, Kevin), Workflow Chairs (Hedayat, Yatin, Dinesh) and Associate Workflow Chairs (Chris, Neil) at AAAI 2021. Many other people contributed to the the conference's design and operation. Notably, Qiang Yang was Conference Chair; Gabriele Röger and Yan Liu were Associate Program Chairs, and Guangneng Hu was a Workflow Chair; all contributed to the design and planning process throughout the year preceding the conference. Even more concretely impacting the content of this paper, Gabi provided draft text on filtering manipulative bids that we adapted into Section \ref{sec:filter-manipulative-bids}, and Yan made contributions to the MIP formulation described in Section \ref{sec: MIP}. The CMT support team provided invaluable real-time service and development during the conference which made our introduction of two-phase reviewing process feasible. Carol Hamilton and the AAAI Office provided innumerable forms of behind-the-scenes support. Finally, an organization as large as AAAI operates only through the efforts of literally thousands of volunteers in myriad roles; we thank \sout{all of them} {\color{blue}the entire AAAI 2021 conference committee and the executives} for their continued service to the community.}


Peer-reviewed conferences, the main publication venues in CS, rely critically on matching highly qualified reviewers for each paper. Because of the growing scale of these conferences, the tight timelines on which they operate, and a recent surge in explicitly dishonest behavior, there is now no alternative to performing this matching in an automated way. 
%
This paper studies a novel reviewer--paper matching approach that was recently deployed in the 35th AAAI Conference on Artificial Intelligence (AAAI 2021), and has since been adopted (wholly or partially) by other conferences including ICML 2022, AAAI 2022, and IJCAI 2022. This approach has three main elements: (1) collecting and processing input data to identify problematic matches and generate reviewer--paper scores; (2) formulating and solving an optimization problem to find good reviewer--paper matchings; and (3) a two-phase reviewing process that shifts reviewing resources away from papers likely to be rejected and towards papers closer to the decision boundary.
%
This paper also describes an evaluation of these innovations based on an extensive post-hoc analysis on real data---including a comparison with the matching algorithm used in AAAI's previous (2020) iteration---and supplements this with additional numerical experimentation.\footnote{Writing this paper and conducting the experimental analysis described herein took almost a full year beyond the conclusion of AAAI 2021. Nevertheless, this paper is grounded in our experiences as Program Chairs (Mausam, Kevin), Workflow Chairs (Hedayat, Dinesh) and Associate Workflow Chairs (Yatin, Chris, Neil) at AAAI 2021. Many other people contributed to the the conference's design and operation. Notably, Qiang Yang was Conference Chair; Gabriele Röger and Yan Liu were Associate Program Chairs, and Guangneng Hu was a Workflow Chair; all contributed to the design and planning process throughout the year preceding the conference. 
Even more concretely impacting the content of this paper, Gabi provided draft text on filtering manipulative bids that we adapted into Section \ref{sec:filter-manipulative-bids}, and Yan made contributions to the MIP formulation described in Section \ref{sec: MIP}. Keshav Sai Kolluru helped in the analysis of the bids, and Shantanu Agarwal helped in coding Subject Area Matching Score (\cref{subsec:SAMS}).
The CMT support team provided invaluable real-time service and development during the conference which made our introduction of two-phase reviewing process feasible. Carol Hamilton and the AAAI Office provided innumerable forms of behind-the-scenes support. The AAAI 2021 conference and executive committees supported us in experimenting with our unconventional ideas for the conference. Finally, an organization as large as AAAI operates only through the efforts of literally thousands of volunteers in myriad roles; we thank all of them  for their continued service to the community. }

==> aaai21_paper_reviewer_matching (5)/bids_processing.tex <==
%\subsubsection{Preprocessing of Bids}
%\label{subsec:bidnorm}
In this section, we describe the techniques we designed for collecting and processing raw data about reviewers and papers into an aggregated score for reviewer--paper matching.
%\m{Maybe give a high level story here, with a diagram.}

\subsection{Calculating Conflicts of Interests} 

A conflict of interest (COI) exists between a reviewer and a paper if the reviewer has a relationship with one or more of the paper's authors that gives them a personal interest in the paper's acceptance or rejection.
%that goes beyond a desire to see high-quality papers get published. 
For example, most of us would struggle to provide a fully unbiased opinion about a paper authored by a former supervisor. Clearly, reviewers should not be matched to  papers with which they have a COI. 

\subsubsection{Filtering Manipulative Conflicts}
Existing reviewer--paper matching systems detect COIs by asking authors and reviewers to disclose all of their current and past affiliations as well as to declare any additional explicit conflicts.
%As mentioned above, users were invited to list other researchers with whom they have a conflict. 
This creates the possibility for a malicious author to provide very long lists of potential conflicts, either in an attempt to lead the system to choose a desired reviewer or simply to avoid expert assessment of their work.
We identified COI declarations as suspicious if they satisfied any of the following criteria: (1) a user listed an unusually large number of email domains as affiliations (8 or more); (2) a user listed an unusually large number of non co-authors as COIs (15 or more); (3) a user self-reported an unusually large number of COIs for which the corresponding reported users did not self-report a reciprocal COI (10 or more). 
We manually examined all such cases and removed all self-declared COIs that did not appear justified on inspecting the user's publicly available profile.
The exact parameters listed above were chosen empirically to capture only extreme behavior: the three conditions respectively captured only (1) 1.1\% of  users who reported more than a one conflict domain; (2) 0.14\% of users who self-reported at least one conflict; and (3) 0.44\% of users with at least one asymmetric conflict. In some cases, we observed evidence of quite egregious behavior: one user reported 35 conflict domains; another reported 57 asymmetric conflicts.  

\subsubsection{Predicting Unreported Conflicts of Interest}
\label{sec: COI}
\input{coi}

\subsection{Filtering Manipulative Bids}\label{sec:filter-manipulative-bids} 
Bids carry important information about reviewers' preferences that can significantly affect reviewers' satisfaction with an assignment. Unfortunately, reviewers can also maliciously submit bids with the aim of affecting a paper's chances of being accepted or rejected \cite{noothigattu2021loss, wu2021making}. 
Most past conferences have tried to detect such misbehavior via Area Chair (AC) oversight, spot checking of discussions, and whistle-blower reports. However, such approaches are labor intensive and scale poorly to huge conferences.

A recent paper \cite{jecmen-etal-neurips2020} proposed alleviating this issue by using a randomized algorithm for the reviewer assignment problem, decreasing the impact of malicious behavior by controlling the probability that certain (suspicious) reviewers or pairs of reviewers are matched to a paper.
However, such randomization can impose significant costs in terms of match quality.
%, and is also difficult to combine with the rest of our MIP formulation.
We nevertheless strongly agree with \citeauthor{jecmen-etal-neurips2020} that malicious behavior is better prevented at the matching phase than detected afterwards. 
We found that the vast majority of papers at AAAI 2021 received a large number of bids by qualified reviewers. As was the case for COIs, the abundance of qualified reviewers allowed us to relatively harmlessly suppress a few potentially suspicious matches even in the likely event that many of them were false positives. 
%\m{Repetition from previous section. Maybe this ethos can move to start of section 2}
%We show here how finer-grained consideration of bidding and assignment structure can dramatically lower the expected benefit of malicious behavior at very low cost to match quality. One strategy we followed was to 
%we asked reviewers to place bids on at least 15 papers. 
At AAAI 2021, bidders could express their level of enthusiasm as \textit{not willing}, \textit{in a pinch}, \textit{willing}, and \textit{eager}.
To reduce the risk of making problematic assignments, we downgraded or suppressed a reviewer's bids when they appeared suspicious, which could happen in a number of ways.

First, a reviewer might place only a few bids to manipulate the likelihood that they would be assigned particular papers (in the most extreme example, bidding positively on only a single paper). To mitigate this risk, we discarded \emph{all} of a Program Committee (PC) member's bidding information if they placed fewer than $9$ positive bids overall (counting \emph{in-a-pinch} bids as half). 
%
We did something similar at other levels of enthusiasm: if a bidder placed fewer than $4$ \emph{eager} bids, we transformed them into \emph{willing} bids; then we transformed fewer than $4$ \emph{willing bids} into \emph{in-a-pinch}. We performed a similar procedure for Senior Program Committee (SPC) members, setting 
a higher threshold of $10$
%higher thresholds
to reflect the higher number of required positive bids.
%Similar to filtering manipulative COI reports, the exact setting of the numbers could vary among different conferences.  
% \nn{Is there any intuition we can give here for these particular numbers of 9 and 4?}
% \klb{State how many times each rule was applied on real bids}

Second, a reviewer could increase their chances of being assigned a particular paper by bidding negatively on many other papers for which they were qualified. We therefore discarded all \emph{not willing} bids of PCs and SPCs if the number of \emph{not willing} bids exceeded six times the number of \emph{willing} and \emph{eager} bids. 

Third, and most complex, \emph{collusion rings} are arrangements under which two or more reviewers agree to positively review each other's papers, a dismaying phenomenon that is reportedly on the rise \cite{littman&al21}. We define two criteria to judge whether a bid by a reviewer $r$ on a paper $p$ is consistent with participation in a collusion ring: (1) at least $40$\% of $r$'s positive bids are on papers authored by 
a specific
%the same
author of $p$; (2) 
there exists some author $r^*$ of $p$ such that both $r$ and $r^*$ bid positively on each other's papers. Specifically, the sum of the number of $r$'s positive bids on papers authored by $r^*$ and the number of $r^*$'s positive bids on papers authored by $r$ is at least $60$\% of 
the total number of positive bids by $r$ and $r^*$. 
For both (1) and (2) above, we considered \emph{eager} and \emph{willing} bids as positive.
%the maximum possible.
%there exists some coauthor $r^*$ of $p$ such that the sum of the number of $r$'s positive bids on papers coauthored by $r^*$ and of $r^*$'s bids on papers coauthored by $r$ is at least $60$\% of the maximum possible.
These criteria are not perfect; e.g., (1) can occur in small subcommunities where a few researchers focus on a given topic, and (2) can wrongly flag reviewers with a few submissions (e.g., two authors with one paper each bid on each other's paper). 
We were willing to tolerate some false positives (for the same reasons outlined above), but aimed to reduce their number by requiring a substantial pattern of suspicious bidding across all of a reviewer's bids. In the assignment process we discarded \emph{all} of a reviewer's bids when 
 either (1) or (2) indicate the reviewer's participation in a collusion ring.

We conducted an extensive manual examination of bids, using various heuristic criteria. In all cases that we judged problematic, our method had already eliminated the appropriate bids.

%\subsection{Constraints to reduce the chances of collusion}


%\cc{Some of these constraints (especially 2-cycle) have the same motivation as some of Gabby's preprocessing in Section 3.2. Include a reference back or reiterate motivation here.}%, undermining \emph{quid pro quo} arrangements in collusion rings.

%\item \textbf{Constraints to reduce the chances of collusion:}



%Finally, we also attempted to rule out assignments that could support collusion directly in our constrained optimization; see below. In brief, our `\textbf{diversity constraints}' prevented multiple, geographically nearby reviewers from casting votes on the same paper, making collusive arrangements harder to set up. Our `\textbf{cycle constraints'} prevented two reviewers from voting on each other's papers, undermining \emph{quid pro quo} arrangements. Both constraints were soft, meaning that they could be violated when enforcing them imposed a nontrivial cost to match quality.

==> aaai21_paper_reviewer_matching (5)/coi.tex <==
\label{sec:COI}
 
Many conference management systems ask users to self-report information such as email domain names for organizations with which the user is currently or was formerly associated. 
Unfortunately, such user-provided information is often incomplete. Users can purposefully withhold information; they can forget to include a past affiliation; and
%For example, affiliation due to an internship might get skipped.
even if they remember every one, they can mistype a domain or fail to report all of their organization's aliases (\eg, \textit{iitd.ac.in} vs \textit{cse.iitd.ac.in}). 
%{\color{blue}Domain normalization and data cleaning, \eg identifying common domain prefixes and suffixes like \textit{.cse, .edu} and \textit{.ac}, 
%can help in mitigating some issues by unifying different aliases of the same organization and hence identifying additional conflicts between users that reported different aliases.
%But obviously such measures cannot detect unreported or incorrect information. 
%}
We performed domain normalization and data cleaning (\eg, identifying common domain prefixes and suffixes, like \textit{.cse, .edu}, and \textit{.ac}, and unifying different aliases of the same organization), but obviously it cannot detect unreported or incorrect information.

%\noindent \textbf{Extracting Conflicts From the Co-authorship Graph:}
We thus augmented user-reported conflicts with additional conflicts based on coauthorship information. We required authors and reviewers to supply DBLP profiles and downloaded the full DBLP database,\footnote{The full DBLP database is publicly available at \textit{\url{http://dblp.uni-trier.de/xml/dblp.xml.gz}}.} allowing us to identify coauthorship relations without the need to disambiguate similar names. We augmented this database with the current conference submissions and built a weighted coauthorship graph, with nodes corresponding to authors, edges existing between pairs of coauthors, and weights representing the number of publications coauthored by the pair.
%We then built a weighted coauthorship graph $G=(V,E)$, where the nodes $V$ correspond to authors, an edge exists between two authors if they appear as coauthors either in a DBLP paper or in a submission to the current conference, and the edge's weight corresponds to the number of such coauthorship relationships between a pair of authors.
% Note that there may exist multiple edges between a pair of nodes, each representing a paper published or submitted jointly by both of them. 
% Each paper written by more than 2 authors, results in multiple labeled edges in the graph: one for each pair of co-authors.
% %The following rules identify a conflict between two nodes in $G$.

One way to prevent COIs would be to prohibit a reviewer from reviewing a paper submitted by a previous coauthor. However, we considered this treatment too strict as it entirely forbids cross reviewing between authors who may not have interacted in years. (Instead, in Section~\ref{sec: constraining_matches}, we describe softer ways in which we discouraged our algorithm from selecting such matchings.) We thus considered a reviewer $r_j$ to have a COI with paper $p_i$ if any of the following conditions were satisfied for some author $a$ of $p_i$: 
%\hz{add something about coauthor constraints here}
\begin{enumerate}
\item $r_j$ coauthored a current conference submission with $a$; 
\item $r_j$ coauthored a published paper with $a$ over the previous 5 years; or 
\item $r_j$ and $a$ coauthored more than 6 published papers over any time period. 
\end{enumerate}
%(1) $i$ coauthored a current conference submission with $j$; 
%(2) $i$ coauthored a published paper with $j$ over the previous five years; or 
%(3) $i$ and $j$ coauthored more than 6 published papers over any time period. 
We further added conflicts between reviewer $r_j$ and papers by an author $a$ when we inferred that $a$ supervised $r_j$ or that both $r_j$ and $a$ were students of the same supervisor. We note that advisor--advisee relationships between users are unknown; hence we need to extract them from the coauthorship graph.
We inferred that $a$ was one of $r_j$'s supervisors if all of the following conditions held:
\begin{enumerate}
\item $a$ began publishing considerably earlier than $r_j$ (at least 5 years);
\item $a$ published at least 10 more papers than $r_j$; and
\item $a$ coauthored many of $r_j$'s early papers (at least 3 out of the first 10). 
\end{enumerate}

These inferences did not need to be perfect: each COI simply prevented a particular reviewer--paper matching, and a few false positive COIs were unlikely to be harmful. Indeed, as we show later in \Cref{fig:qualified} (\Cref{sec: scoring_function_evals}), most papers had a large number of highly qualified reviewers, indicating that occasionally forbidding one of them was unlikely to materially affect the quality of the matching.

%provided there were multiple qualified reviewers to choose from for a given paper.

We observe that we are not the first to use DBLP to infer COIs; \citet{long&al13} describe methods for inferring coauthor, colleague, advisor--advisee, and competitor relationships. Like us, they used DBLP data to identify coauthor relationships. However, they relied on users' public web pages to identify colleague and advisor--advisee relationships. We did not consider the latter approach feasible given the large scale of AAAI 2021. 
% \begin{comment}
% Notes From the google doc:
% (1) Between every two authors compute DBLP co-authorship based COI:
% Disregard papers with more than 7 authors
% If two people co-authored a paper in last five years COI = 1
% If two people co-authored more than 6 papers together at any time COI = 1
% If Person 1 is senior to Person 2 and they co-authored several early papers of Person 2, COI = 1. (Here the guess is that Person 1 is the advisor)
% We could conceivably also say that Person 2 has COI with all co-authors of Person 1… not sure if it becomes too extreme.
% Else COI = 0

% (2) Between every two authors COI = 1 if one of the authors expressed COI explicitly or with the email domain
% As an exception we will look at self-reported COIs, and check manually if
% A user has an unreasonable number (8) of domains  as COI domains 
% A user has an unreasonable number (15) of non co-authors as COIs 
% A user has a large number of self-reported COIs (10) where the COIs’ don’t have this user as a COI in their self-reports
% (3) Between each pair of co-authors in AAAI 2021 submissions, declare COI=1
% (4) If COI between two people is 1, then COI between one and papers written by the other is also 1
% \end{comment}

==> aaai21_paper_reviewer_matching (5)/conclusion.tex <==
This paper has presented a novel method for reviewer--paper matching that is scalable to large conferences and more robust to malicious behavior. Our formulation is based on a mixed-integer program that combines a scoring function (which itself combines three match scores and reviewer bids) with various soft constraints encouraging the optimizer to pick, for each paper, a set of reviewers that is geographically diverse, includes at least one senior reviewer, and does not include co-authors. Several preprocessing steps predict new conflicts of interest alongside known ones, and reviewer bids are also processed to undermine malicious bids. A Two-Phase reviewing scheme uses available reviewing resources more efficiently by allocating fewer reviews to papers that have low acceptance probability. We performed extensive evaluation and post-hoc analysis to demonstrate the value of our methods. We have publicly released our reviewer--paper matching software for further use by other conferences, and indeed this software is already in use at ICML 2022. Furthermore, the two-phase reviewing methodology and various other novel elements of the design described here have been adopted by AAAI 2022 and IJCAI 2022. 


==> aaai21_paper_reviewer_matching (5)/constraining_matches.tex <==
We formulated the problem of maximizing our scoring function subject to our set of both hard and soft constraints as a Mixed-Integer Programming (MIP) problem. 
%We formally state our MIP in Section~\ref{subsec: MIP_def}.
It is quite natural to formulate the
%~\cite{lian&al18,kobren&al19,tang&al10,flach&al09,taylor&al08,garg&al10}. 
reviewer--paper matching problem as one of maximizing an aggregate weighted matching score subject to reviewer and paper capacity constraints and avoiding COIs, and much past work has done so  \cite{flach2010novel,garg&al10,tang&al10,lian&al18,taylor&al08,kobren&al19,charlin&al13,charlin&al11}.  
Indeed, with only COI and capacity constraints, this formulation corresponds to a network flow problem and is thus solvable in polynomial time~\cite{taylor&al08}. 
%However, it is known that finding a matching using this simple program would end up with poor matching outcomes such as skewness in the reviewers' workload or an unbalanced distribution of expert reviewers among related papers~\cite{kobren&al19}. 
Unfortunately, that formulation can yield an inequitable distribution of work across reviewers and of scores across papers.
To address this, \citet{stelmakh2019peerreview4all} and \citet{kobren&al19} focused on finding more balanced matchings.  Specifically, instead of the common objective of maximizing the aggregate weighted matching score,  \citet{stelmakh2019peerreview4all} look into finding matches that maximize the minimum matching score across all papers. Because the resulting optimization problem is NP-hard, they design an approximation algorithm, which finds a suboptimal solution by solving a series of network flow problems. \citeauthor{kobren&al19}---like us---aim to maximize an aggregate weighted matching score, but took a somewhat different approach. Specifically, they augmented an Integer Linear Program with lower and upper bounds on the assignments per reviewer and also added local fairness constraints to ensure that the total matching score for each paper would exceed a threshold; they propose an approximation algorithm that relaxes integrality constraints to solve their assignment problem. Our own approach uses slack variables to soften hard constraints instead of relaxing the integer constraints, resulting in a mixed-integer program. 
We also introduce a wide range of additional constraints. 
We now describe our approach in more detail.

\subsection{Constraining Matches}
\label{sec: constraining_matches}

It would not suffice simply to identify a score-maximizing matching: the best reviewers could be given hundreds of papers; different papers could receive very different treatment, leading to an unfair assignment. For example, a paper may get assigned all junior reviewers from one research group. 
%\hz{I am not sure if I like using unfair here, without defining it}
%\yn{The line following it gives an example of being unfair. Should be ok I guess.}
%would be unnecessarily vulnerable to manipulation via malicious behavior. 
We thus imposed various \emph{constraints} on reviewer--paper matchings.

%The first three are quite straightforward. The fourth constraint ensures that experienced reviewers are distributed fairly across papers. This may assist the reviewing process in multiple ways. For example, it may help in streamlining the discussions amongst reviewers, in addition to exemplar training of the first time reviewers. 

%Our two phase reviewing process requires assigning \textit{unbiased} and \textit{qualified} reviewers to evaluate submitted papers at each phase. 
%The goal of reviewer--paper-Assignment problem is to assign \textit{unbiased} and \textit{qualified} reviewers to evaluate submitted papers. 

% We formulate the problem as a Mixed-Integer Program (MIP), adding constraints , where the objective function, $\obj$, captures the \textit{quality} of the reviewer--paper match and the constraints ensure that the match is \textit{unbiased}.
% Unlike past works that have also used ILP formulation for PRA, our novel constraints not only guarantee that all papers are assigned sufficient reviewers, but also attempts to: 1) prevent malicious behaviour, 2) assign independent reviewers to a paper, with at least one senior reviewer, and 3) ensure equitable load amongst reviewers.

% \noindent \textbf{Objective Function:} The quality of a reviewer--paper match is quantified via a novel scoring function, $\scorematrix$, that combines four different sources of information: 1. reviewer bids, 2. declared subject areas of both reviewers and  papers, 3. standard TPMS scores \citep{charlin&al13}, and finally, 4. a neural scoring function based on similarity of the submitted paper with the published works of the reviewer: we call it ACL Score \footnote{ACL Score has been developed recently by the ACL conference organizers: https://acl2020.org/blog/conflict-of-interest/}. 
% %We describe our scoring function in detail in
% See \cref{subsec: MIP_score} for details on scoring function.

%\newcommand{\constraint}[1]{\vspace{.3em}\noindent\textit{#1.}~}
\newtheorem{constraint}{Constraint}

\begin{constraint}[COI] 
\label{cons:coi}
No reviewer should be assigned to a paper with which they are in conflict.\end{constraint}

\begin{constraint}[Number of Reviewers]
\label{cons:numreviewers}
Each paper must receive a specified number of reviews. 
\end{constraint}
Historically, this number of reviews has been three at AAAI and many other AI conferences. In our  two-phase reviewing system (see Section~\ref{sec: two-phase}) we solved the reviewer--paper matching problem separately in each of our phases, assigning two reviewers for each paper in Phase 1, 
and adding additional reviewers in Phase 2 such that each paper not rejected in Phase 1 got at least four reviews across the two phases. (That is, we added extra reviewers in Phase 2 when reviewers didn't submit their reviews at the end of Phase 1.)

\begin{constraint}[Reviewer Load]
\label{cons:reviewerload}
The number of papers assigned to any reviewer should not exceed some maximum. 
\end{constraint}
At AAAI 2021 we had a hard limit of three papers per reviewer per phase, and (as we will discuss later) penalized matchings that assigned more than two papers per reviewer in a given phase.

%\vspace{.3em}

%\begin{constraint}[Seniority]
%Each paper is assigned at least one experienced reviewer. Our goal was to ensure that experienced reviewers were distributed fairly across papers, to reduce variance in reviews, ensure that each discussion had at least one experienced participant, and thereby aid in the training of novice reviewers. 
%\end{constraint}

\begin{constraint}[Seniority]
\label{cons:seniority}
Each paper is assigned at least one experienced reviewer. 
\end{constraint}
Our goals were: (1) to ensure that experienced reviewers were distributed fairly across papers; (2) to reduce variance in reviews; and (3) to ensure that each discussion had at least one experienced participant, to promote the training of novice reviewers. 

A second set of constraints served both to ensure that each paper is reviewed by an intellectually diverse set of reviewers and to make collusion rings harder to sustain. Collusion is only possible amongst reviewers who can somehow communicate with one another. By preventing pairs of co-authors from reviewing the same papers,  preventing arbitrary pairs of reviewers from bidding to review each other's papers, and by choosing reviewers from as diverse a set of geographic regions as possible, we limited opportunities for gaming the system.
% having independent opinions from reviewers assigned to each paper is beneficial for the review process in large conferences
 %\hz{added something about the benefit of having independent reviewers}

\begin{constraint}[Coauthorship Distance] 
\label{cons:coauthor}
No two reviewers assigned to the same paper have small distance in the coauthorship graph.
\end{constraint}

\begin{constraint}[Geographic Diversity]
\label{cons:geo}
No two reviewers assigned to the same paper belong to the same geographic region. 
\end{constraint}
%We inferred regions based on academic affiliations and email addresses. 

\begin{constraint}[No 2-Cycles]
\label{cons:cycle}
No pair of reviewers who both bid positively on each other's papers may review each other's submissions. 
\end{constraint}
% \yn{I have added a note in the 2-cycles constraint. Not sure if this is the best way to put it.}

\vspace{.3em}
It would not have been desirable to satisfy these constraints at all costs. 
For many papers, it was easy to find qualified reviewers satisfying all of these constraints; however, for others imposing all of these constraints would dramatically have degraded reviewer quality or even made it impossible to find the required number of reviewers.
For example, qualified reviewers often bid on each other's papers without harboring malicious intent. Out of caution, we adopted the principle of finding matchings that avoided such cases when reasonable alternatives were present, but were willing to relax the principle otherwise. We therefore expressed all but \textit{COI},  \textit{Number of Reviewers}, and PC's \textit{Reviewer Load} as soft constraints. More specifically, for each constraint we identified a constant expressing its importance and penalized the objective function by this constant each time the constraint was violated for a reviewer--paper pair. Observe that the task of identifying these constants was dramatically simplified by our decision to normalize our scoring function between $0$ (worst possible reviewer--paper matching) and $1$ (best possible matching). For example, expressing a coauthorship distance penalty of $0.1$ would mean that we would prefer to accept a reviewer--paper matching scoring up to $0.1$ points lower in exchange for satisfying the constraint.


==> aaai21_paper_reviewer_matching (5)/intro.tex <==
\setcounter{footnote}{1}
% Peer-reviewed conferences, the main publication venues in CS, rely critically on matching highly qualified reviewers for each paper. Because of the growing scale of these conferences and the tight timelines on which they operate, there is now no alternative to performing this matching in an automated way. 
% %
% %With the unprecedented scale of the conferences, it is not possible to manually match reviewers to the papers and hence to ensure fair and equitable assignment of reviewers to the papers, creating an unbiased automated matching process becomes crucial.
% %
% %This paper proposes a suite of methods for matching papers with reviewers that maintain high quality standards, ensure fairness, and reduce the effectiveness of various forms of malicious behavior. 
% %
% %
% O

%This not only violates the double blind policy, but also the conflict of interest and exposes the malicious intent of the participants in the collusion ring, maligning the entire process of peer-review.
%Peer-reviewed conferences, the main publication venues in CS, rely critically on matching highly qualified reviewers for each paper. Because of the growing scale of these conferences and the tight timelines on which they operate, there is now no alternative to performing this matching in an automated way. 

%9,034 submissions
%This paper describes and analyzes the novel, automated reviewer--paper matching approach that debuted at the 35th AAAI Conference in Artificial Intelligence (AAAI 2021). 
Submissions to prominent AI conferences have grown steadily in recent years. The AAAI Conference on Artificial Intelligence (AAAI) received fewer than 1,000 submissions in each of its first 33 years (1980--2012); fewer than 2,000 submissions annually until 2015; and fewer than 4,000 submissions annually until 2018. AAAI 2021 received over 9,000 submissions! Program committees have grown to keep pace with submissions; nearly 10,000 reviewers were involved in the 2021 conference. Given the scale and the tight timeline on which such large conferences operate---roughly three months between paper submission and author notification---it is becoming an increasingly challenging problem to assign reviewers\footnote{Modern conference reviewing is often divided into four hierarchical roles, though terminology can vary. At AAAI, Program Committee members (PCs) review submissions; Senior Program Committee members (SPCs) facilitate discussions among PCs and write meta-reviews; Area Chairs (ACs) oversee the review process, communicate with SPCs about final decisions, and recommend accept/reject decisions; Program Chairs design and oversee the whole review process and make final decisions for each submission. In this paper, we sometimes use the term reviewer to refer exclusively to PCs; in other cases, we refer to PCs, SPCs, and ACs. Distinctions between the two cases should nevertheless be clear from the context.} to papers about which they can provide high-quality reviews. Some key subproblems are estimating how qualified a given reviewer is to review a particular paper; tractably finding good matchings; determining which papers can be rejected without full review; and identifying reviewers who have bid, reviewed, or scored papers in an attempt to manipulate outcomes. 
%.\cc{I revised above sentence but still needs some work. Crucial sentence but tricky to write.}

%With the unprecedented scale of the conferences, it is not possible to manually match reviewers to the papers and hence to ensure fair and equitable assignment of reviewers to the papers, creating an unbiased automated matching process becomes crucial.
%
%This paper proposes a suite of methods for matching papers with reviewers that maintain high quality standards, ensure fairness, and reduce the effectiveness of various forms of malicious behavior. 
%
% Ensuring that our reviewing mechanisms continue to function well is critical to the continued health of our field.
%\m{What is our contribution? Is it: 
%A new system? 
%Specific technical pieces?
%An integrated solution for paper reviewing?
%}
We addressed these challenges with a novel automated pipeline for reviewer--paper matching at AAAI 2021. Our pipeline consists of three main elements: (1) collecting and processing input data to identify problematic matches and generating reviewer--paper scores; (2) formulating and solving a constrained matching problem; and (3) splitting the reviewing process into two phases to better allocate reviewing resources towards borderline papers. We briefly describe each of these in turn (and then devote a full section to each in what follows). Code for our pipeline is available at \url{https://github.com/ChrisCameron1/LargeConferenceMatching}.%In the recent past, many authors have complained on social media about poor quality of reviews, reviews going unchecked even by Senior Program Committee members and Area Chairs, demonstrating either a dearth of good reviewers, or issues with the existing reviewer--paper matching systems.\nn{Citation needed}


%\m{As written, the contribution of this part is a bit Unclear.}
\newcommand{\minipar}[1]{\vspace{6pt plus 6pt}\noindent\textbf{#1.}~}
\minipar{Data Collection and Processing} Program Chairs need to transform a reviewer's profile into an estimate of how qualified that reviewer is to review each paper. Profiles can be as detailed as Program Chairs are creative, containing features such as
%identities, 
past email addresses,  DBLP/Semantic Scholar profiles, self-reported reviewing proficiency via a bidding phase, self-declared conflicts of interest (COIs), and texts of previously written papers. A key question that conference organizers need to answer is how to process this data and transform it into a numerical score assessing the quality of every plausible reviewer--paper pair. Two notable examples of such numerical scores are TPMS~\cite{charlin&al13} and ACL scores~\cite{neubig&al20}. 
Both of these scores are computed based on textual similarity between a submitted paper and reviewer's prior publications. However, they are not always available; TPMS scores can only be computed for reviewers whose prior publications are known and ACL scores can only be computed for reviewers whose past publication abstracts are accessible, e.g., via a known Semantic Scholar profile. 
In AAAI 2021, we computed TPMS and ACL scores for all applicable reviewer--paper pairs. We also knew 
%users'
reviewers' and papers'
primary and secondary subject areas and received explicit bids from reviewers. We aggregated all of our data to obtain final reviewer--paper scores that were between 0 and 1 and whose values were unbiased by missing data. We refer to the resulting scoring function as \emph{aggscore}. 

Input data is only as useful as it is trustworthy: a rising concern for large scale conferences is that %reviewers
participants
may self-report information to direct their submission to a specific reviewer or to ensure they review a specific paper
\cite{jecmen-etal-neurips2020}.
%Most past conferences have tried to detect such misbehavior via Area Chair (AC) oversight, spot-checking of discussions, and whistleblower reports. However, such approaches are labor-intensive and not particularly effective. %A recent paper \cite{jecmen-etal-neurips2020} proposed alleviating this issue by using a randomized algorithm for the reviewer assignments problem, which decreases the impact of malicious behavior by controlling the probability that certain (suspicious) reviewers or pairs of reviewers are matched to a paper.
%However, such randomization can impose significant costs in terms of match qualities.%, and is also difficult to combine with the rest of our MIP formulation.
%We nevertheless agree with \citeauthor{jecmen-etal-neurips2020} that malicious behavior is better prevented at the matching phase than detected afterwards. In our approach, 
To that end, we constructed relationship graphs based on each 
%reviewer's 
user's
publication history to identify unreported conflicts (which, of course, also arose via mistakes or oversights from non-malicious users). We also developed a set of heuristics to identify suspicious patterns of self-reported conflicts and of bidding for papers to review. In both cases, we erred on the side of being cautious, forbidding all such suspicious assignments.

% \textit{Calculating Conflicts of Interests:} 
% When assigning papers to reviewers, a reviewer that has conflict of interest with a paper (e.g., due to their relationship with the authors) cannot give an impartial review to the paper \nn{Rephrase to define COI}. Therefore, such reviewer--paper pairs must be avoided. Existing reviewer--paper matching systems rely on authors and reviewers themselves to report the information required to calculate their conflicts of interest. This creates an opportunity for a malicious author to provide a very long list of potential conflicts so that either the system would end up choosing a desired reviewer or every expert who can give an accurate assessment of the work is eliminated. To avoid this dishonest behavior,  we propose running a data analysis of the COI declaration data. Then, conference organizers should manually check users that seemed suspicious and removed unjustified COI declarations. In AAAI 2021, this approach was deployed and the most extreme examples that we found were 35 domains reported and 57 self-reported asymmetric conflicts \nn{I don't think there's enough context to understand this sentence. I might leave it out. No one knows what an assymetric conflict is, for exmaple}.

% Based on the following phenomenon we have not left our COI calculation for AAAI 2021 there : even if a user attempts to honestly and completely report their affiliations, such user-provided information is often incomplete, e.g., COIs can be missed if a user mistypes any domains or if an organization has many different aliases \nn{I would stop here until ``Therefore'' and leavae the rest to the relevant section} (\eg, \textit{iitd.ac.in} and \textit{ cse.iitd.ac.in} both represent \textit{Indian Institute of Technology Delhi}, but a participant may not provide both). Some of these issues can be handled through domain normalization and data cleaning (\eg, identifying common domain prefixes and suffixes, like \textit{.cse, .edu, .ac}), but these will not solve the issue of missed conflicts due to unreported or incorrect information. Therefore, we required authors and reviewers to provide us with their DBLP profiles. \nn{This related work belongs out of the intro and in the section IMO} We were not the first to use DBLP to infer COIs; \citet{long&al13} describe methods for inferring coauthor, colleague, advisor-advisee, and competitor relationships. Like us, they use DBLP data to identify coauthor relationships, but rely on users' homepages to identify colleague and advisor-advisee relationships. We did not consider the latter approach feasible given the large scale of AAAI 2021. Instead, we automatically extract users' coauthorship relationships from the list of their publications on DBLP. Overall, our data analysis shows that 3.6\% of the total conflicts in AAAI 2021 were detected via DBLP, which corresponds to at least one additional conflict to a large majority (78.8\%) of submissions. 



% \textit{Pre-processing of the Bids:} In many CS large conferences, reivewers are asked to bid on papers. These bids are a way for reviewers to show their preferences \nn{I would not say preferences - reviewers are supposed to bid for papers they are qualified to review, not ones they ``feel'' like reviewing} over the papers and can affect their satisfaction with the assignment significantly. Unfortunately, reviewers can adopt several strategies to maliciously misreport bids: a reviewer may place few bids in total or may bid negatively on many papers for which they are qualified to increase their chances that they are assigned a particular paper that they intend to review. Furthermore, reviewers can form \emph{collusion rings} through bidding, which is to positively review each other's papers, a dismaying phenomenon that is reportedly on the rise \cite{littman&al21}. To avoid such bad behavior, we propose asking reviewers to place bids on at least a certain number of papers \nn{Our innovation is the bid transformation, not the requirement to bid on X papers.}. Then, deploy a bid transformation process to filter manipulative bids. %For example, we discarded “all" of a reviewer's bidding information if they placed fewer than 9 positive bids overall. 
% In AAAI 2021, we asked reviewers to bid on at least 15 papars. Upon using this approach, we found that that the vast majority of papers in our conference received a large number of bids by qualified reviewers, making suppressing a few potentially suspicious matches relatively harmless even if they are false positives. \hz{missing evaluation data from Gabi}



% \textit{Scoring reviewer--paper pairs:} a key challenge for any automated reviewer--paper matching is quantifying the value of matching. It is critical to get this right: readers may recall that our initial matching at AAAI 2021 had to be recalled because we miscalibrated our scoring function---based on the emails we received, reviewers definitely noticed.

% \nn{I do not think this belongs in the intro} There is a body of work on automatically discovering latent topics of a submission and comparing it with latent topics of a set of papers authored by a given reviewer \citep{mimno&al07, long&al13, anjum&al19, kobren&al19, wieting&al19}. A paper by \citet{conry&al09} proposes a score based on the primary and secondary subject areas of the paper and that of the reviewer, embedding both reviewers and papers in a discrete vector space 
% %$K^{N_\psi}$, where $N_\psi$ is the total number of topics, $K = \{-1/2, 0, 1/2, 1\}$, 
% with each discrete dimension quantifying the affinity of the reviewer (paper) to the corresponding topic. The TPMS score  \cite{charlin&al13} is computed based on the similarity between the text of a submitted paper and a reviewer's prior publications. 
% %The similarity is quantified by the dot product between a paper vector and a reviewer vector. 
% The ACL matching score \cite{neubig&al20} compares abstracts of a submitted paper and the abstracts of a reviewer's prior publications in a dense vector space.
%is computed based on the textual similarity between abstract of a submitted paper and abstracts of reviewer's prior publications,
%; code is available at \url{github.com/acl-org/'-matching}.
%The abstract representation is computed by averaging the embeddings of subwords generated by sentencepiece~\cite{kudo-richardson-2018-sentencepiece}.%\nn{What is a subword embedding?}
%\citep{wieting&al19}. 
 %A score is computed for each of the reviewer's prior publications with respect to the paper. The top three scores are aggregated to compute the ACL score. 
%As TPMS score is based on topics in the text, it represents paper/reviewer at a higher level of abstraction, whereas ACL score is based on words in abstracts and hence it represents paper/reviewers at a much lower level of abstraction.
%Each reviewer was requested to provide their Semantic Scholar ID and links to their prior publications. We profile each reviewer by extracted abstracts from these two sources. 
%The ACL matching score is same as the score used for reviewer matching in ACL conferences. The only difference is that we train the scorer using abstracts of papers published in past AAAI and related conferences rather than abstracts from ACL anthology. 
% TPMS scores can only be computed for reviewers whose prior publications are known and ACL scores can only be computed for reviewers whose past publication abstracts are accessible, e.g., via a known Semantic Scholar profile. 
% Match qualified reviewers to submissions. We score each (paper, reviewer) pair in a way that aggregates many sources of information and is robust to missing data. Specifically, we combine scores based on keyword agreement with scores based on textual similarities with a reviewers' prior publications (TMPS, ACL).

% In AAAI 2021, we had access to TPMS and ACL scores whenever they were available for any reviewer--paper pair. We also knew users primary and secondary subject areas. Our goal was to combine this information to find an aggregated score that more reliable than using any of the individually available scores and is robust to missing data. Missing data was a real concern for us because reviewers had to manually provide the information required to compute these scores, and thus many reviewers had at least once missing entry. In fact, 3.36\% and 39.75\% of users were missing TPMS and ACL scores, respectively. Therefore, we designed a new way to score reivewer-paper pairs, that is robust to missing data. We first computed a so called Subject Area Matching Scores (SAMS) which is an extension of discrete affinity scores to continuous ones in a way that captures more information. Then, we normalize raw TPMS, ACL and SAMS scores to make sure that they have the same scale and merged them together. Finally, we accounted for reviewers bids and cleaned up low scoring matches to avoid the possibility of wildly inappropriate matches. Our data analysis on AAAI 2021 data shows that our aggregated score is high for any \nn{I doubt for any is true} reviewer--paper pair which has gotten a positive bid by the reviewer. This is a strong evidence for us that our scoring function indeed captures expertise. Furthermore, our analysis showed the robustness of our scoring function to missing data; For any given paper, the standard deviation of the changes in aggregated scores caused by missing data were around 0.05, whereas the mean standard deviation of the complete-data score was 0.117. \nn{This is too complicated a result to say in the intro. You have to either summarize it in a vague but still true way and link to a section or not say anything. This isn't clear at all}



\minipar{Formulating a Constrained Matching Problem} Once scores have been assigned, the next key problem is to come up with an actual assignment. We formulated this problem as a Mixed-Integer Programming (MIP) problem. We are far from the first to use a MIP formulation for reviewer--paper matching~\cite{flach2010novel,garg&al10,tang&al10,lian&al18,taylor&al08,kobren&al19,charlin&al13,charlin&al11}. However, we went well beyond the vanilla ``find a score maximizing assignment'' formulation by including additional (soft) desiderata. For example, we penalized assigning coauthors to review the same paper, rewarded geographic diversity in assignments, and penalized assignments where reviewers each bid positively on each other's papers. These soft constraints served both to ensure that each paper was reviewed by an intellectually diverse set of reviewers and to make potential collusion rings (reviewers conspiring to review each other's papers) \cite{littman&al21} harder to sustain.
Separately, we introduced a seniority constraint to encourage our matching algorithm to distribute experienced reviewers across papers. 
%{\color{blue}Our experimental analysis shows that these soft constraints only marginally impacted the mean aggregate score. Hence they did not significantly degrade average match quality while making it difficult for the users to game the system.}
We show in our experimental analysis that despite the mentioned advantages, these soft constraints only marginally impacted the mean aggregate score, and hence did not significantly degrade average match quality.

To ensure that the resulting MIP formulation could be solved within a reasonable amount of time, we sparsified our space of possible assignments by creating variables representing the possibility of assigning a given paper to a given reviewer only when the pairing had a sufficiently high score; we then used column generation as necessary to identify further candidate reviewers for hard-to-match papers. Our coauthorship constraints were too large to specify in memory, and so we similarly leveraged row generation (i.e., we identified an initial solution without coauthorship constraints and then iteratively added individual violated constraints and reran the optimization). See~\Cref{fig:flow_diagram} for how the information flows through our reviewer assignment system.


%In addition to filtering malicious reports, we induced soft constraints that penalize assignments with the potential to facilitate malicious behavior: close colleagues reviewing the same paper, and authors reviewing each other's papers.
% We are far from the first to formulate the
% %~\cite{lian&al18,kobren&al19,tang&al10,flach&al09,taylor&al08,garg&al10}. 
% reviewer--paper matching as the problem of maximizing an aggregate weighted matching score subject to reviewer and paper capacity constraints and avoiding COIs  \cite{flach&al09,garg&al10,tang&al10,lian&al18}.  
% With only the COI and capacity constraints, this formulation corresponds to a network flow problem and is solvable in polynomial time~\cite{taylor&al08}. 
% %However, it is known that finding a matching using this simple program would end up with poor matching outcomes such as skewness in the reviewers' workload or an unbalanced distribution of expert reviewers among related papers~\cite{kobren&al19}. 
% \nn{Again, this RL really gets in the way of the intro flow}
% However, that formulation can yield an inequitable distribution of work across reviewers and matching score across papers.
% To address this, some recent work has focus on finding more balanced matchings~\cite{stelmakh2019peerreview4all, kobren&al19}. Notably, \citet{kobren&al19} augmented their optimization problem with local fairness constraints ensuring that the total matching score for each paper is above a threshold; they propose an approximation algorithm that relaxes integrality constraints to solve their assignment problem. Our own approach introduces a wide range of additional constraints and uses slack variables to soften various hard constraints instead of relaxing the integer constraints, resulting in a mixed-integer program. In addition to COI and reviewer and paper capacity constraints \nn{You haven't defined these}, we have a set of seniority constraints which ensures that experienced reviewers are distributed fairly across papers. %This may assist the reviewing process in multiple ways. For example, it may help in streamlining the discussions amongst reviewers, in addition to exemplar training of the first time reviewers. 
%In addition to filtering malicious reports, we induced soft constraints that penalize assignments with the potential to facilitate malicious behavior: close colleagues reviewing the same paper, and authors reviewing each other's papers.

%Collusion is only possible amongst reviewers that can communicate with one another; by preventing coauthors from reviewing together or each other's papers and by further trying to segregate reviewers by region, we limit opportunities for gaming the system.
% having independent opinions from reviewers assigned to each paper is beneficial for the review process in large conferences
 %\hz{added something about the benefit of having independent reviewers}
 










% We optimize these scores via a scalable Mixed-Integer Programming (MIP) formulation that also rewards geographic diversity among coreviewers, light reviewer workloads, and an even spread of senior reviewers across papers. We note, however, that we are far from first to adopt this perspective: much related work has studied different aspects of the reviewer--paper matching problem. To streamline exposition, the paper is organized topically, with related work discussed in each section.


\minipar{Two-Phase Reviewer Assignment} The quality of papers submitted to conferences like AAAI 2021 varies vastly. Reviews are signals of quality, but can be very noisy. This was perhaps most convincingly demonstrated via an influential NeurIPS experiment \citep{lawrence&al17}, which split reviewing between two independent Program Committees. The experiment found that while the strongest and weakest papers could be reliably identified, many papers close to the decision boundary were accepted by one Program Committee and rejected by the other. This finding invites the idea of obtaining additional reviews for papers close to the decision boundary to reduce variance, and points out that one way to obtain this additional reviewing capacity is to reduce the reviewing load allocated to papers far below threshold.

%In the years since, many conference organizers have  reallocate reviewing resources from papers that are nearly certain to be rejected to papers that have a realistic chance of acceptance.
%\begin{figure}[ht]
\begin{wrapfigure}{r}{0.6\textwidth} 
\centering
% \usetikzlibrary{shadows,arrows.meta,positioning,backgrounds,fit,chains,scopes}
% \resizebox{0.6\textwidth}{!}{\input{figures/flow_diagram.tikz}}
%\includegraphics[width=0.6\textwidth]{figures/FlowDiagram2Colored3.pdf}
\includegraphics[width=0.5\textwidth]{figures/tikz_cropped_final.pdf}
\caption{Schematic diagram showing the flow of information in our system. %Data sources are used to compute various  Conflict Of Interests (COIs). In addition to this, filtered bids are used to compute the aggregate score (aggscore) between (paper,reviewer) pairs. 
%COIs, aggscores, and filtered bids, along with other inferred information such as seniority, geographic region of a reviewer, and co-authorship distance between two reviewers, are used to create an MIP formulation for the task of Paper-Reviewer Matching. Finally, the formulated MIP is solved using \Cref{alg:itersolve} that first instantiates appropriate number of variables using column generation and then iteratively calls row (constraint) generation to assign the desired number of reviewers to each paper.
}
\label{fig:flow_diagram}
\end{wrapfigure}
%\end{figure}
One commonly used approach in journals which has also been adopted by recent AI conferences such as IJCAI 2020~\cite{bessiere&al20} summarily rejects some fraction of papers without full reviews (based, e.g., on quick perusal of each paper by one or more Area Chairs). However, this approach can be difficult to implement fairly (Area Chairs may not have strong opinions after a quick perusal; some papers will be missed; and such an approach would still impose a huge workload across 9,000 submissions). Even when it works well, the approach still leads to poorly explained decisions that many authors find frustrating (a quick perusal does not result in a detailed justification for the decision or suggestions about how work can be improved). 

We used an alternative to summary rejection, which we refer to as \textit{Two-Phase Reviewing}. This approach has various historical antecedents; we defer a survey of those to Section~\ref{sec: two-phase}. Roughly, instead of assigning, say, three reviews to each paper, we initially only assign two. If the two reviews agree that a paper should be rejected, the paper is indeed rejected without further reviews. A second phase of review assignments allocate two additional reviews to the papers that remain.  This approach redirects reviews to borderline papers while also giving meaningful feedback (two full reviews) to authors of rejected Phase 1 papers, and avoids the overhead of a separate summary rejection phase by treating all papers in the same way. It also has various other benefits. Notably, it gives Program Chairs a second opportunity to assign additional reviewers for papers identified as problematic or for which Phase 1 reviewers went missing; and also facilitates mechanisms like AAAI's ``NeurIPS/EMNLP FastTrack", in which high-scoring rejected papers from sister conferences with late notification dates are allowed to proceed directly to Phase 2, with their reviews from the sister conference taking the place of Phase 1 reviews.

%-------------------------------------------------
% From Michael Littman
%
% Thanks for reaching out. Here's what we wrote about it in the CFP. As you can see, the goal wasn't reviewing efficiency but a concern that some papers were being rejected simply because they weren't fully understood by the reviewers. I'm pretty sure it was Leon's idea (he's very creative that way) and should be the one to comment on any inspirations he drew on.
%
% Review Process (New for 2009!)
% Our review process this year will be slightly different from previous years to further encourage innovative papers on a variety of topics. Authors will indicate a preference for an Area Chair to handle their papers (see the list of Area Chairs). The goal here is to ensure each submission is considered by reviewers appropriate to the paper's intended contribution. Each submitted paper will receive two first round reviews. As in recent years, authors will have the opportunity to see and respond to the reviews before a final decision is made. Papers that receive at least one positive review in the first round will receive one or more additional reviews. Final decisions will be made using the input from all reviewers, the author feedback, the Area Chair, and Program Chairs. Reviewing for ICML 2009 will be blind to the identities of the authors. No conditional accepts will be granted this year.
%-------------------------------------------------

%-------------------------------------------------
% From Leon:
%
% ICML'09 was small by today's standards but the community was growing at a large pace. Therefore the number of trusted reviewers –I mean here reviewers that the Area Chairs know and trust—was small in regards to the number of submissions.  During the first phase of the review, the papers were routed to Area Chairs and reviewers whom we expected would be sympathetic to the paper.  So if they all find the paper wanting, it didn't make much sense to allocate trusted reviewers for further reviews.
%
% In parallel we had a special sessions "Food for thought" with papers with high variance reviews. These were typically papers in which some reviewers recognized a substantial novel idea but that other reviewers found insufficiently polished.  The default processes tend to reject those papers, but we wanted them accepted because we believe that bringing new ideas, however unpolished, is one of the goals of a scientific conference.  This is of course hit or miss. Interestingly one of these five or six papers collected >3500 references, and another one about 200.
%
% There was a meeting around the end of the conference where we discussed the outcome of the process. I could not find the slides or the survey. I remember that the two-stage process did not cut a large fraction of the total number of reviews. On the other hand, it forced the Area Chairs to look at their allocated papers twice instead of once :-)  Whether this has helped reach better outcomes is hard to say.  The Program Chairs of ICML'10 decided to return to a conventional process because the two stage process left very little time for author responses and discussion.
%
% Hope it helps.
%
% Leon
%-------------------------------------------------


% {\color{red} While we designed our Two-Phase approach independently, we have subsequently realized that various versions of the idea have been implemented at CS conferences over at least the past dozen years. To our knowledge, the first conference to use two reviewing phases was ICML 2009~\cite{Bottou}/ 
% % The chairs' motivations were similar---high variance in some reviews and a desire to make reliable choices---but re were some key differences, however. One chair explained to us that ``the goal wasn't reviewing efficiency but a concern that some papers were being rejected simply because they weren't fully understood by the reviewers.''\footnote{This and subsequent quotes were obtained via personal communication with the ICML 2009 Program Chairs, Leon Bottou and Michael Littman.}  Indeed, the other chair elaborated that ``the two-stage process did not cut a large fraction of the total number of reviews.'' this problem was driven by the community's rapid growth and the difficulty of told us that ``ICML'09 was small by today's standards but the community was growing at a large pace. Therefore the number of trusted reviewers –--I mean here reviewers that the Area Chairs know and trust---was small in regards to the number of submissions.  During the first phase of the review, the papers were routed to Area Chairs and reviewers whom we expected would be sympathetic to the paper.  So if they all find the paper wanting, it didn't make much sense to allocate trusted reviewers for further reviews.''
% %
% % The Program Chairs of ICML'10 decided to return to a conventional process because the two stage process left very little time for author responses and discussion.
% %
% though it was later abandoned by ICML 2011's Program Chairs as it involved manual allocation of Area Chair's which became difficult with the increasing size of the conference.
% %\st{due to the increasing size of the conference and its tight timeline.}\nn{This is a weird excuse to make, given that we adopted it for a large conference with tight timelines}\cc{Agreed. Can we be sure this is this reason ICML stopped? If so, is it because they had more manual work needed. I would cut if we can't make more precise.}
% %\yn{Quoting from ICML09's chair's response: "\textit{The Program Chairs of ICML’10 decided to return to a conventional process because the two stage process left very little time for author responses and discussion.}". But you are right:  I think the main cause is the manual allocation of ACs}
% Outside of AI, at least a few conferences in the systems community have also adopted Two-Phase reviewing; we're aware of XXXX \cite{Hans}, YYY \cite{Adve2010} and ZZZZ \cite{Adve2014}.

%We have independently come up with the Two-Phase idea and implemented it in large scale for the first time.
% To the best of our knowledge, at its time, AAAI 2021 represented the largest implementation of Two-Phase reviewing in a scientific conference.
% Our approach was maintained by AAAI 2022 and has also been adopted by IJCAI 2022 and ICML 2022. }
%\cc{Add citations and reframe novely of two-phase}

We also describe the impact of these for AAAI 2021.
%\ycom{Rephrase the 1st line?}
%The reader may wonder how this all worked out at AAAI 2021. 
2,615 %\todo{Yatin: or 2615 as in the opening remarks? Also check the footnote. Feel free to edit}
papers (37\%)\footnote{Out of 9071 abstract submissions in Phase 1, only 7133 were accompanied by a full paper, out of which 37\% were rejected in Phase 1.} received two high-confidence reviews recommending rejection and so were rejected in Phase 1, which gave us a surplus of 2,615 %\todo{Yatin: or 2314, as in the 2nd line of this para, we say that usually 3 reviewers are assigned, and in phase 1, we have utilized 2 of them?}
reviews (relative to AAAI's previous practice of assigning 3 reviews to every paper) to spread among the remaining papers in Phase 2 and FastTrack submissions. In AAAI 2021, the FastTrack received 778 abstract submissions and 688 full paper submissions, out of which 268 were ultimately accepted.
%Of course, a key question is {\color{blue} how} well the method avoids rejecting papers in Phase 1 that would ultimately have been accepted if they received four full reviews? 
A key question is whether the rejected papers in Phase 1 would ultimately have been accepted if they received four full reviews. We devote Section~\ref{sec: evaluations} to an extensive real-data analysis that investigates such questions, but for this one (examined in detail in Section~\ref{sec:false-negatives}) we give a brief synopsis here. We identified an (inadvertent) natural experiment: when papers did not receive two full, high-confidence reviews in Phase 1, we promoted them to Phase 2 regardless of their scores and assigned additional reviewers. By subsampling pairs of reviews from the larger set that these papers eventually received, we estimate that there was only a 2.9\% probability that a Phase 1 rejected paper would eventually have been accepted to AAAI 2021. 

% \klb{Stats on fast-track submissions and acceptances?}
% \begin{itemize}
%     \item Match qualified reviewers to submissions
%     \item behavior
%     \item Balancing the resources
%     - Minimize reviewer effort spent on obvious rejects
%      - Give more attention to borderline papers
%     \item Diversifying the resources
%     \item Robustness in the acceptance side
%     \item Support NeurIPS fast track
% \end{itemize}

%

%NN:9961 reviewers counting PC/AC/SPC for all tracks and AISI


The remainder of this paper is organized as follows. We begin by describing the details of our approach for data collection and processing in \Cref{sec: input}. Then, we present our mixed-integer programming formulation of the reviewer--paper matching problem %and show how it can be approximately solved even for very large conferences using row generation
in \Cref{sec: MIP}. We describe our Two-Phase reviewing scheme %that shifts reviewing resources away from papers that are nearly certain to be rejected and towards papers on the decision boundary
in \Cref{sec: two-phase}. \Cref{sec: evaluations} consists of an exhaustive experimental analysis of data from AAAI 2021 in which we deployed these methods. Finally, we summarize our contributions in \Cref{sec: conclusion}. We note that much related work has studied different aspects of the reviewer--paper matching problem. To streamline exposition, we discuss related work in each corresponding section.
%This paper begins by  When then describe an approach for automatically augmenting conflict of interest declarations (Section~\ref{sec: COI}) and filtering out manipulative reports about both conflicts and bids to review papers (Section~\ref{sec: bids_processing}). We then describe methods for scoring the quality of prospective reviewer--paper matches, ultimately proposing a novel approach that combines keyword declarations, methods for assessing similarity between a submission and a reviewer's past work, and reviewer bids into a single normalized score (Section~\ref{sec: scoring_function}). We identify a wide range of constraints on matches, some of which we soften into penalties on the objective (Section~\ref{sec: constraining_matches}).  The remainder of the paper consists of an exhaustive experimental analysis of data from AAAI 2021 in which we deployed these methods, analyzing the effectiveness of our two-phase reviewing design (Section~\ref{sec: two_phase_evals}), match quality (Section~\ref{sec: scoring_function_evals}), and the scalability of our MIP solution techniques (Section~\ref{sec: MIP_scalability_evals}).


% \begin{itemize}
%     \item We describe the methods used to run AAAI 2021, a conferrence involving X reviewers and Y papers.
%     % \item One challenge is scale: approaches that work for conferences with hundreds of submissions break down when both papers and reviewers number in the thousands. 
%     % \item Another challenge is a recent surge in explicitly dishonest behavior such as collusion rings, where authors collude to bid on each others' papers with the goal of submitting fraudulent reviews \cite{littman&al21}. 
%     % \item We aim to convince the reader that both of these problems can be mitigated by the application of AI techniques, assessing the usefulness of our methods on real data from the 35th AAAI Conference in Artificial Intelligence (AAAI 2021). For example, x papers were submitted to AAAI in 2021, as compared to only y in AAAI-2015. (See https://www.openresearch.org/wiki/AAAI)

    
% \end{itemize}



==> aaai21_paper_reviewer_matching (5)/new_commands.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{soul}           %strikethrough
\usepackage{amssymb}       % math symbols


\usepackage{amsmath}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\usepackage{array}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}
\usepackage{amsmath}% http://ctan.org/pkg/amsmath
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\usepackage{graphicx}
\usepackage{graphics}

\usepackage{comment}
\usepackage{soul} 
\usepackage{listings}
\usepackage{float}
\usepackage{placeins}
\usepackage{subcaption}
\usepackage{wrapfig,lipsum,booktabs}
\usepackage{natbib}
\usepackage[normalem]{ulem}
\usepackage{bbm}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{appendix}
\usepackage{cleveref}

%\usepackage{lineno}
%\linenumbers
%  \usepackage{titling}

%\usepackage{draftwatermark}
%\SetWatermarkText{Draft Do Not Distribute}
%\SetWatermarkScale{0.5}
%\SetWatermarkLightness{0.9}



\usepackage[algo2e]{algorithm2e}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{accents}
%\usepackage{algpseudocode}
%\usepackage[table,xcdraw]{xcolor}

\usepackage{thmtools,thm-restate}
\usepackage{enumitem}

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{cor}{Corollary}

%\usepackage{calrsfs}
\usepackage{xcolor}

\newcommand{\mcom}[1]{{\color{brown}{{[M: #1]}}}}
\newcommand{\ycom}[1]{{\color{red}{{[Y: #1]}}}}
\newcommand{\notsure}[1]{{\color{orange}{{[Y: #1]}}}}

\newcommand{\TT}[1]{\mbox{\tt #1}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\BE}{\begin{enumerate}}
\newcommand{\EE}{\end{enumerate}}
\newcommand{\etal}{\mbox{\it et al.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\cf}{\mbox{\it cf.}}
\newcommand{\Eg}{\mbox{\it E.g.}}
\newcommand{\Ie}{\mbox{\it I.e.}}
\newcommand{\?}{\mbox{?}}


\DeclareMathOperator{\Lagr}{\mathcal{L}}
\DeclareMathOperator{\EX}{\mathbb{E}}% expected value

% \newcommand\shortcite{\citeyearpar}
\newcommand\newcite{\citet}
\renewcommand\cite{\citep}	
%\let\oldhat\hat

%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\renewcommand{\vec}[1]{\mathbf{#1}}
%\renewcommand{\hat}[1]{\oldhat{\mathbf{#1}}}
%\newcommand\Set[2]{\{\,#1\mid#2\,\}}

\newcommand{\fourpartdef}[8]
{
	\left\{
		\begin{array}{llll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4 \\
			#5 & \mbox{if } #6 \\
			#7 & \mbox{if } #8 \\
			
		\end{array}
	\right.
}



\newtheorem{definition}{Definition}

\newcommand{\pluseq}{\mathrel{+}=}

\newcommand{\xscore}{S_{(x)}}
\newcommand{\tpmsscore}{S_{t}}
\newcommand{\aclscore}{S_{a}}
\newcommand{\sascore}{S_{s}}

\newcommand{\nxscore}{Sn_{(x)}}
\newcommand{\ntpmsscore}{Sn_{t}}
\newcommand{\naclscore}{Sn_{a}}
\newcommand{\nsascore}{Sn_{s}}

\newcommand{\assignmat}{\mathbf{X}}

\newcommand{\assignmatentry}{x}


\newcommand{\papers}{\mathcal{P}}
\newcommand{\reviewers}{\mathcal{R}}
\newcommand{\pcs}{\mathcal{PC}}

\newcommand{\spcs}{\mathcal{SPC}}
\newcommand{\acs}{\mathcal{AC}}
\newcommand{\obj}{O}
\newcommand{\matchingscore}{S}
\newcommand{\scorematrix}{S}
\newcommand{\scorematrixentry}{s}

\newcommand{\subjectareas}{\Psi}
\newcommand{\subjectarea}{\psi}

\newcommand{\primarysubjectarea}{\mathbb{P}_\psi}
\newcommand{\secondarysubjectarea}{\mathbb{S}_\psi}

\newcommand{\primarypapersubjectarea}{\mathbb{P}}

\newcommand{\capacity}{c}
\newcommand{\capacityentry}{c}
\newcommand{\lowerlimitcapacity}{l}
% \newcommand{\capacityslack}{\mathbf{SL_{cap}}}
\newcommand{\capacityslack}{s^{\text{cap}}}

\newcommand{\capacityslackpenalty}{p^{\text{cap}}}

% \newcommand{\cyclevars}{\mathbf{SL_{cy}}}
% \newcommand{\cyclepen}{Pen_{cy}}

\newcommand{\cyclevars}{s^{\text{cy}}}
\newcommand{\cyclepen}{p^{\text{cy}}}

\newcommand{\cycles}{CY}

% \newcommand{\seniorityslack}{\mathbf{SL_{sen}}}
% \newcommand{\seniorityreward}{\text{Reward}_{sen}}

\newcommand{\seniorityslack}{s^{\text{sen}}}
\newcommand{\seniorityreward}{\text{Reward}^{\text{sen}}}

% \newcommand{\numregion}{\mathbf{Reg}}
\newcommand{\numregion}{\text{reg}}
% \newcommand{\paperregion}{\mathbf{PR}}
\newcommand{\paperregion}{v}
\newcommand{\region}{r}
\newcommand{\regions}{\text{Regions}}
% \newcommand{\reviewerregion}{RR}
\newcommand{\reviewerregion}{t}
\newcommand{\regionreward}{\text{Reward}^\text{reg}}

% \newcommand{\coauthordist}{Co}
\newcommand{\coauthordist}{d}

% \newcommand{\coreview}{\mathbf{Cor}}
\newcommand{\coreview}{\text{cad}}
\newcommand{\coreviewerset}{V}

\newcommand{\coimat}{\text{COI}}
\newcommand{\coimatentry}{\text{coi}}


\newcommand{\constraints}{\mathcal{C}}






==> aaai21_paper_reviewer_matching (5)/scoring_function.tex <==

%A scoring function quantifies how good a reviewer is for a submitted paper.
A key question in automated reviewer--paper matching is quantifying the value of matching a reviewer $r_j$ with a submitted paper $p_i$, which we denote as $\scorematrixentry_{ij}$.
It is critical to get this right.\footnote{Indeed, a few readers may remember that our initial matching at AAAI 2021 had to be changed, and the reason was that we accidentally miscalibrated our scoring function. Based on the emails we received, reviewers definitely noticed!}
In brief, we considered a match to be good if the reviewer both had expertise in the paper's subject matter and was interested in the paper. We assessed expertise by aggregating three complementary signals: Toronto Paper Matching System (TPMS) scores; ACL matching scores; and degree of match between the paper's primary and secondary subject area keywords and those of the reviewers. We assessed degree of interest via bids, assuming a baseline level of interest for papers about which a reviewer was predicted to have expertise and for which the reviewer did not submit any explicit (positive or negative) bid.


Much existing work has leveraged similar signals, much of which is focused on automatically discovering latent topics of a submission and comparing it with latent topics of a set of papers authored by a given reviewer \citep{mimno&al07, long&al13, anjum&al19, kobren&al19, wieting&al19}.
Three further lines of related work deserve detailed discussion, since we either extended them \cite{conry&al09} or leveraged them directly \cite{charlin&al13,neubig&al20}. 

First, \citet{conry&al09} proposed a score based on the primary and secondary subject areas of the paper and that of the reviewer. The fundamental idea was to embed both reviewers and papers into a discrete vector space 
%$K^{N_\psi}$, where $N_\psi$ is the total number of topics, $K = \{-1/2, 0, 1/2, 1\}$, 
with each discrete dimension quantifying the affinity of either the reviewer or the paper to the corresponding topic. 

Second, the TPMS score  \cite{charlin&al13} is computed based on the similarity between the text of a submitted paper and a reviewer's prior publications. 
The similarity is quantified by the dot product between a paper vector and a reviewer vector. The paper vector is constructed using the topic proportions in the text of the submitted paper identified by Latent Dirichlet Allocation (LDA) \cite{blei&al03}. The reviewer vector is computed by taking an average of the topic proportions in each of the reviewer's prior publications.
TPMS scores can only be computed for reviewers whose prior publications are known. 

Third, the ACL matching score \cite{neubig&al20} compares abstracts of a submitted paper and the abstracts of a reviewer's prior publications in a dense vector space.
%is computed based on the textual similarity between abstract of a submitted paper and abstracts of reviewer's prior publications,
%; code is available at \url{github.com/acl-org/'-matching}.
The abstract representation is computed by averaging the embeddings of subwords generated by the SentencePiece tokenizer \cite{kudo-richardson-2018-sentencepiece}. %\nn{What is a subword embedding?}
%\citep{wieting&al19}. 
 A score is then computed for each of the reviewer's prior publications with respect to the paper. The top three scores are aggregated to compute the ACL score. 
%As TPMS score is based on topics in the text, it represents paper/reviewer at a higher level of abstraction, whereas ACL score is based on words in abstracts and hence it represents paper/reviewers at a much lower level of abstraction.
%Each reviewer was requested to provide their Semantic Scholar ID and links to their prior publications. We profile each reviewer by extracted abstracts from these two sources. 
%The ACL matching score is same as the score used for reviewer matching in ACL conferences. The only difference is that we train the scorer using abstracts of papers published in past AAAI and related conferences rather than abstracts from ACL anthology. 
ACL scores can only be computed for reviewers whose past publication abstracts are accessible, e.g., via a known Semantic Scholar profile. 

The rest of this section is organized as follows. We first describe how we computed Subject Area Matching (SAM) scores, a continuous extension of discrete affinity scores. Then, we describe how we normalized raw TPMS, ACL and SAM scores to make sure that they have the same scale. We then explain how we merged these scores to make them robust to missing data. This was a real concern because we needed to rely on reviewers to manually provide the information required to compute these scores, and around 40\% of the reviewers had at least once missing entry. Next, we explain how we adjusted these scores to take into account reviewers' bids. Finally, we describe an approach for pruning low-scoring matches, which we used to avoid the possibility of wildly inappropriate matches.

\subsubsection{Subject Area Matching Score (SAM)}
\label{subsec:SAMS}
We scored the keyword match between papers and reviewers via an extension of the affinity scoring idea described earlier \cite{conry&al09}, which embeds each reviewer and paper in a %continuous 
% Dinesh: @yatin it should be continuous space - right?
%{\color{blue} discrete}
vector space. Our approach went beyond explicitly specified subject areas by learning correlations between different keywords. This is important because the approach of \citet{conry&al09} assigns a weight of 0 to keywords that are not specified explicitly, even when these have a strong degree of semantic similarity with a keyword that \textit{is} specified. 
For example, keywords \textit{``Humans and AI -> Human-Agent Negotiation"} and \textit{``Game Theory and Economic Paradigms -> Negotiation and Contract-Based Systems"} were highly correlated at AAAI 2021, and thus it might be inaccurate to assign a weight of $1$ to only one of the two when the other is absent.

%\todo{Yatin: please proof-read this paragraph once for grammatical correctness.}
%\klb{Give an example of two keywords we considered very correlated.})
% {\color{blue}
\input{appendix}
% }
%\sout{We call the result \textit{Subject Area Matching Score (SAM Scores)}.} 

% Copied from the previous version: The scoring function ensures (1) paper's primary area contributes more than all the secondary areas, (2) the more the number of secondary areas match, the higher the score, and (3) papers do not get penalized for providing fewer (or zero) secondary areas.

Some intuitive properties of SAM scores are: it considers the primary keyword to be more important than all of the secondary keywords; gives each individual keyword less weight when more keywords are listed; and imputes additional keywords (with lower weights) for reviewers based on keyword co-occurrence patterns across the whole conference. 
%\sout{The details of the SAM scores calculation are presented in  \Cref{sec: Appendix}.}

%The full definition of SAMS appears in Section~\ref{subsec: SAMS}.

%\yn{In the previous version, we had the mathematical details/definition of SAMS in the appendix. Those details are completely missing from this version. I think we should put them back.}

%We now discuss how the paper vectors and the reviewer vector are computed. Each subject area $\subjectarea$ can be expressed as $\text{parent}(\subjectarea) -> \text{child}(\subjectarea)$. For example, in the subject area \textit{NLP} $->$ \textit{Dialog Systems}, \textit{NLP} is the parent and \textit{Dialog Systems} is the child. Each parent subject area can have multiple child subject areas.Each submission and reviewer have one primary subject area ($\primarysubjectarea$) and multiple secondary areas ($\secondarysubjectarea$).

%\subsection{TPMS Score}


%Each reviewer is expected to create a TPMS profile and upload prior publications. 
%As TPMS is integrated with the conference management toolkit, the scores are fetched by sending the submission PDFs and the list of reviewers to TPMS.
%Hence, 
%This score can only be computed for reviewers who have setup their profile in TPMS.

%\subsection{ACL Matching Score}


\subsubsection{Normalizing Scores}
We wanted all final scores to lie in the range $[0,1]$ so that we could use consistent units to set the parameters that penalize violations of soft constraints (e.g., we might penalize violation of a soft constraint by $0.1$ units, meaning that we would accept a match that scored $0.09$ units worse in order to preserve the constraint, but not a match that scored $0.11$ units worse).
Since we computed the three component scores (TPMS, ACL and SAM) independently, and since we observed a huge discrepancy between the numerical range of the three raw scores, we first normalized them each individually before taking their weighted average as the final matching score.

%both TPMS and ACL scores were missing for many reviewers, it was easier to combine scores when each component score (TMPS, ACL and SAMS) was first normalized to the same range. 
%
To do so, for each score, we independently and randomly selected many (paper, reviewer) pairs. A Program Chair manually examined each pair (reading the paper's abstract and the reviewer's profiles) and annotated each pair $(p_i,r_j)$ as $y_{ij} \in \{1, 0.75, 0.5, 0\}$, corresponding to \textit{excellent}, \textit{good}, \textit{in-a-pinch}, and \textit{bad} matches respectively. We then performed a linear regression mapping the raw score component to $y_{ij}$ and clipped the resulting function to the range $[0,1]$.

% To normalize, we regress $y_m$ independently on the three raw scores: let $f_t(.), f_a(.) \text{and} f_s(.)$ be the three independently learnt (linear) predictors of $y_m$ using the TPMS, ACL and Subject Area matching scores.
% We then simply use $f_t, f_a$, and $f_s$, clipped between $0$ and $1$, as the normalization functions for the three scores: $\nxscore[i,j] = \max\{0,\min\{1,f_{(x)}(\xscore[i,j])\}\}$, where 
% $\xscore[i,j]$ and $\nxscore[i,j]$ are raw and normalized scores respectively, and 
% $(x)= t, a,$ and $s$ for TPMS, ACL and Subject Area scores respectively.

% Note that another alternative is to regress $y_m$ on all the three scores together: that would take care of their aggregation as well.
% But unfortunately, the coverage of the three scores is highly non-uniform with one or more score missing for many (paper, reviewer) pairs. Besides, while aggregating, we want to carefully select their weights, especially when the final matching score is below a threshold.
% Hence, we decide to first normalize them independently and then aggregate using manually assigned weights to each score.

% \begin{comment}
% Before we combine the three scores to compute the final matching score, we first need to ensure that they are all comparable. 
% However, we observed a huge discrepancy between the numerical range of the three raw scores.
% Hence, we first normalize them before taking their weighted average as the final matching score.
% We manually tagged around 50 to 100 data points and fit a piece-wise linear curve between the raw score and the self-assigned score. 
% We assign a score of 1, 0.75, 0.5 and 0 for an excellent, good, in-a-pinch, and a bad match respectively.
% The normalized scores were clipped between 0 and 1.
% For ACL, 
% We first observe that bottom 90\% of all the three match scores are going to be insignificant: this is expected as one reviewer would know only about a couple of subject areas, and hence his matching score with submissions in rest of the subject areas is expected to be low.
% For each of the three scores, we randomly select $10,000$ (paper, reviewer) pairs from the top 10\%. 
% We further divide the $10,000$ samples in to $10$ buckets based on their score. Within each bucket, we randomly select 5 to 10 samples and manually assign a score 
% \end{comment}

% \subsubsection{Score Aggregation:}
\subsubsection{Aggregating Scores} 
\label{subsec:scoreagg}
Our next task was to aggregate scores into a single number between $0$ and $1$, in a way that was robust to missing TPMS and ACL scores. We decided to give more weight to keyword-based scores than either of the automatically inferred scores (TPMS and ACL), since keyword scores were computed using information provided explicitly by authors and reviewers. %\hz{how about reliable instead of interpretable?}
When both TPMS and ACL were present, we summed TPMS + ACL + 2 * SAM and then renormalized; when only one of TPMS and ACL were present, we summed the 
%remaining 
 available
score and SAM score and renormalized; when only SAM score was present we used it as the base aggregated score:
\begin{equation*}
\text{Base Aggregated Score} =\begin{cases} \frac{1}{4}\text{TPMS} + \frac{1}{4}\text{ACL} + \frac{1}{2}\text{SAM} & \text{if all data is present} \\
\frac{1}{2}\text{ACL} + \frac{1}{2}\text{SAM} & \text{if TPMS is missing} \\
\frac{1}{2}\text{TPMS} + \frac{1}{2}\text{SAM} & \text{if ACL is missing} \\
 \text{SAM} & \text{if both ACL and TPMS are missing}
\end{cases}
\end{equation*}


% The purpose of score aggregation is to provide a unified objective function, representing the overall quality of a match, which is ultimately maximized by the MIP for the assignment.
% Unfortunately, we can't simply add the three normalized scores for a (paper, reviewer) pair, as their coverage is highly skewed, and for most of the pairs one or more scores are missing.
% In addition, we chose to assign a higher weight to the subject area scores, .
% Hence, we propose the following aggregation function which takes care of the missing scores (N.A.) appropriately:
% \begin{equation*}
% \begin{aligned}
% \scorematrix[i,j] &= 0.50\nsascore[i,j] + 0.25\ntpmsscore[i,j] + 0.25\naclscore[i,j]   \\
% =& 0.50\nsascore[i,j] + 0.50\ntpmsscore[i,j]  \ \text{if} \ \naclscore[i,j] = \text{N.A.}\\
% =& 0.50\nsascore[i,j] + 0.50\naclscore[i,j] \ \text{if} \ \ntpmsscore[i,j] = \text{N.A.} \\
% =& 1.00\nsascore[i,j] \ \text{if} \   \ntpmsscore[i,j] = \naclscore[i,j] = \text{N.A.}\\
% =& 0.00 \ \text{if} \   \nsascore[i,j] = \ntpmsscore[i,j] = \naclscore[i,j] = \text{N.A.}
% \end{aligned}
% \end{equation*}

%Notice that the TPMS and ACL scores are not available ($N.A.$) for all the reviewer--paper pairs, and hence our aggregation function takes that into account appropriately.

\subsubsection{Accounting for bids} Given this score capturing reviewer \emph{expertise}, we still needed to account for reviewer \emph{interest} as expressed through bidding to obtain a final result we called \emph{aggscore}. We computed aggscore by upweighting/downweighting the base aggregated score based on the bid. Our approach to combine expertise and interests does not allow bids to override the base aggregated scores. We achieved this by computing aggscore as follows:
\begin{align*}
    \rm{aggscore}=(\rm{Base~aggregated~score})^{\rm{bidscore}}
\end{align*}
We used bidscores as $20, 1, 0.67, 0.4, 0.25$ corresponding to \textit{not-willing, not-entered, in-a-pinch, willing, and eager} bids, respectively.
% Next, we need to encourage an assignment when a reviewer bids positively for a paper and conversely, we need to discourage an assignment for which reviewer has explicitly mentioned his unwillingness.
% Accordingly, we modify the final score based on the bids of the reviewers as
% %\begin{equation}
% %\label{eq:bidexponent}
% $
% \scorematrix[i,j] = \scorematrix[i,j]^{1/\alpha},
% $
% %\end{equation}
% where $\alpha = 0.05, 1.00, 1.50, 2.50,$ and $4.00$ for a \textit{not-willing, not-entered, in-a-pinch, willing, and eager} bid respectively.
% Such a transformation amplifies the reviewers' preference while ensuring that the transformed score remains within $0$ and $1$.
% This is crucial for setting up the penalties for different constraint violations: we exactly know how much score are we trading off per violation.
Observe that this procedure maintained scores in the range between $0$ and $1$; exponents greater than $1$ (for \emph{not-willing}) reduced scores while exponents less than $1$ (for \emph{in-a-pinch, willing,} and \emph{eager}) increased scores. Our use of an exponent of $1$ for papers that received no explicit bid left those scores unchanged.
% When the reviewer bid is positive ($\alpha > 1$), it increases a low matching score (and vice-versa) and the quantum of increase (or decrease) depending on how far $\alpha$ is from $1.0$.
%the exact bid value.
% It also ensures that the score remains the same when the bid is \textit{not-entered} ($\alpha = 1.0)$.
%While making bidding collusion rings,  reviewers tend to bid only on very few papers, thereby inflating their matching scores and hence the likelihood of  
%Please see section \cref{subsec:bidnorm} for details on various steps w
Observe also that our use of exponentiation (as compared e.g., to adding a constant and renormalizing) meant that reviewers could not influence the system to give them papers for which they were manifestly unqualified, whereas the presence or absence of a bid could make a significant difference to the scores of sufficiently qualified reviewers.

\subsubsection{Cleaning up low scoring matches} Finally, we observed that while high ACL or TPMS scores indicated good matches, their assignment of low values carried much less signal than low SAM scores. Hence, when aggscore was less than $0.15$, we used the minimum of $0.15$ and the SAM score exponentiated by the reviewer's bid.
% %\begin{equation}
% $
% \scorematrix[i,j] = \min \{\nsascore[i,j]^{1/\alpha}, \gamma\} \ \ if \ \ \scorematrix[i,j] \le \gamma. 
% %\end{equation}
% $
This transformation ensured that whenever a low-scoring match was selected, it was at least from the same subject area. This avoided the possibility of wildly inappropriate matches and helped reviewers see some rationale for our decisions to assign poorly matching papers.



\begin{comment}

When nk is available
0.25*(ntpms + nacl) + 0.5*nk when all three available
0.5*ntpms + 0.5*nk when nacl is NA
0.5*nacl + 0.5*nk when ntpms is NA
nk if both ntpms and nacl are NA

When nk is not available
0.5*(ntpms + nacl) when both available
ntpms  when nacl is NA
nacl when ntpms is NA
0 if both ntpms and nacl are NA

fs = s**(1/alpha) where alpha = 0.05,1,1.5,2.5,4
[not willing, not entered,in a pinch, willing eager ]

if fs <= 0.15 , then we want to backoff to subject area score which is most interpretable.
fs  = min(nk**(1/alpha), 0.15)
\end{comment}


%\subsection{The formal definition of the Subject Area Matching Score (SAMS)}
%\label{subsec: SAMS}


==> aaai21_paper_reviewer_matching (5)/scoring_function_evals.tex <==
%\subsection{Matching quality analysis}
We deployed the reviewer--paper matching approach described above for the AAAI 2021 conference. In this section, we analyze a dataset of 6,729 submissions\footnote{For this analysis we removed papers that were withdrawn, desk rejected, or rejected as dual submissions. We also excluded all papers from the AI for Social Impact track as these papers were matched via a somewhat different process. We included papers that were only submitted in the second phase.}, 
the specific reviewer matching we obtained for them,
and 
the resulting paper
%\sout{and their} 
%\hz{I don't see how the new wording is making things more clear} 
reviews
from 8,072 reviewers in the main conference's PC\footnote{In AAAI 2021, Program Chairs, ACs, and SPCs manually assigned about 4.5\% of the final reviewer assignment. In fact, many of these were suggested by area chairs in Phase 2 based on the reviews in Phase 1. In our evaluations, we only considered matches that were automatically assigned to avoid confounding factors of manual matches.}. Unfortunately, we are unable to release the data used for any analyses because data about a conference review process is inherently sensitive, but we summarize our findings in what follows.
%\hz{@Yatin, please fact check this paragraph below}
%\yn{@Neil, could you please check the number of reviewers?}
We used the following parameters\footnote{The values of these parameters express tradeoffs between violating a constraint and match quality, and hence induce the reviewer--paper matching problem's objective function. There is no ``right'' way to set them: they reflect Program Chairs' subjective answers to questions like the value of having senior reviewers allocated to each paper and the risk of authors forming bidding cycles. This paper does not experimentally investigate these parameter settings, but we note that other conference organizers could conceivably want to set them differently.} (see Section~\ref{subsec: MIP_def} for definitions): $\regionreward = 0.1$, $|\regions|=5$, $\cyclepen = -0.05$, $p^\text{co}(1) = -0.3$, $p^\text{co}(2) = -0.2$, $\seniorityreward = 4$, $\text{TargetSeniority}=4$, $\text{MinSeniority}=0$. In Phase 1, we set reviewer capacities to 3 for PCs, and set $\gamma_\text{pc} =2$, $\gamma_\text{spc} = \gamma_\text{ac} = 1$; we increased PC capacity to 4, and set $\gamma_\text{pc} =4$, $\gamma_\text{spc} = \gamma_\text{ac} = 0$ in Phase 2. We only made assignments to SPCs and ACs in Phase 1 except for the fast track papers for which we set $\gamma_\text{spc} = \gamma_\text{ac} = 1$. We set reviewer capacities to 24 and 60 for SPCs and ACs respectively. We set $W=5$ with $\capacity_{j\cdot}= [8,12,16,20,24] \forall j \in \spcs$ and $\capacity_{j\cdot}= [20,30,40,50,60]$ for $j \in \acs$, with $\capacityslackpenalty_w(\cdot)=-0.05, 1 \le w \le (W-1)$ and a very high penalty of $-0.5$ for $\capacityslackpenalty_W(\cdot)$ for both SPCs and ACs, so that the system never assigned beyond $\capacity_{jW}=\capacity_j$. 
%\klb{I've tried to ensure that phrases used in math mode aren't italicized here and in the previous section. Make sure I didn't introduce inconsistencies---the multiple file hierarchy prevents easy searching.}


%\nn{I tried to write something here to ward off similar hyperparameter arguments, feel free to delete - I'm not convinced it works}
%klb: moved to a footnote up



We begin by asking whether we made good matches in the real conference. Before we begin our analysis, we note that evaluating match quality is conceptually tricky. Of course, the gold standard is to ask Area Chairs to manually ensure that matchings make sense; it is also possible to monitor social media for outrage \cite{lawrence_2014}. Our focus here was to go beyond such subjective measures, performing a data-driven and quantitative evaluation along as many dimensions as possible. What follows is, to our knowledge, the most comprehensive post-hoc evaluation of a Computer Science conference's match quality. (Indeed, we note that such analyses are usually limited only to the graphs that appear in Program Chairs' presentations at conference business meetings. Of course, the confidentiality of reviewing data typically prevents others from conducting further, in-depth analyses.)
%\cc{Heddy TODO: cite paper saying this is hard question}

% 2.00    0.074522
% 4.00    0.348876
% 6.00    0.419870

\begin{figure*}
    \centering
    \includegraphics[width=.6\textwidth]{figures/confidence_scores}
    \caption{Paper score distribution by confidence of reviewer. More confident reviewers gave fewer 5s and 6s.\label{fig:confidence_v_score}}
\end{figure*}
\begin{figure*}
    \centering
  \includegraphics[width=.6\textwidth]{figures/confidence_v_aggscore}
    \caption{Reported confidence of an eventual review vs. predicted aggscore for all reviewer--paper pairs matched at AAAI 2021.\label{fig:confidence_v_aggscore}}
\end{figure*}


%   \subfigure[Scores for phase-two papers computed using all reviews (x-axis) and using all combinations of 3 reviews (y-axis). Any given paper could receive very different scores depending on the subset of reviewers it received.\label{fig:aaai_score_variance}]{\includegraphics[width=0.65\columnwidth]{figures/score_variance}}
% \end{figure*}

\subsubsection{Did our scoring function capture reviewer expertise?} First, we investigated whether reviewers actually bid on papers for which we assigned them high ``expertise'' scores, leveraging the fact that reviewers tend to bid positively on papers that they are capable of reviewing. 
Considering the set of reviewers who submitted at least one bid, we looked at all matched reviewer--paper pairs that we assigned base scores (i.e., aggscores before taking bids into account) greater than $0.75$. We found that 29\% of these pairs were accompanied by \textit{eager} bids, 38\% \textit{willing}, and 3\% \textit{in a pinch} (the remainder no bids). 
We see this as evidence that high base scores indeed correlated with high match quality. However, we acknowledge that the bidding interface is a possible confounding factor here---e.g., users could view papers in descending order of  their TPMS scores (one of the inputs to aggscore).
%\klb{I rephrased to be clearer about what you filtered on. Make sure I didn't introduce an error.}

Second, we observe that the distribution of overall scores given by reviewers to papers (which ranged between 1 and 10) noticeably changed as a function of self-reported confidence.\footnote{Confidence levels could be reported as ``Reviewer made an educated guess'', ``Reviewer is broadly knowledgeable, but not an expert in the area'', ``Reviewer is knowledgeable in the area of the paper'', or ``Reviewer is an expert in the specific topic of the paper''.} Figure \ref{fig:confidence_v_score} shows that more confident reviewers tended to give more informative paper scores (fewer borderline 5 and 6 scores). Given that higher confidence reviews were more informative, we examined the relationship between our scoring function and reported reviewer confidence. Figure~\ref{fig:confidence_v_aggscore} shows that our scoring function was positively correlated with confidence: as confidence increased, so did the 25th, 50th, and 75th percentile of scores.
% 
\subsubsection{Assuming that our scoring function predicted review quality, how close did we come on average to assigning the best possible reviewer to each paper?}
% \cc{We consider matches that were automatically assigned to avoid confounding factors of manual matches. This represents 95.5\% of the dataset described above.}
We considered the ordinal ranking of reviewers assigned to each paper in terms of aggscore, where rank 1 corresponds to the reviewer with the highest aggscore for that paper. We then looked at the mean reviewer ranking for each paper with respect to the ranks of all of the paper's reviewers.
The first / second / third quartiles of mean reviewer rankings across all papers were 7 / 12 / 28. This shows that papers were often assigned very highly qualified reviewers; note that these averages are taken across all of a paper's reviewers (median 4) and that a single reviewer with a poor rank is able to cause the average ranking to grow large.

% TOD): What about the rank according to reviewers. Not as important but still interesting.
% TODO: Put this into context of k=50. We don't allow many matches with > 50 rank. (must be at most rank 50 according to paper or reviewer)


% NN - In light of the fact that region constraints seem to have been disabled in the actual matching for most of the areas we discuss, we probably want to ditch this section
% \subsubsection{In which subject areas were soft constraints most violated?}
% A large fraction of soft constraint violations---notably for the geographic diversity and coauthorship constraints---occurred in only a few subject areas. We suppress their particular identities for anonymous peer review but will describe them in the full version of this paper.
%In particular, the proportion of reviews from duplicated regions (geographic constraint violations) were highest in \emph{Knowledge Representation and Reasoning} (0.49) and \emph{Constraint Satisfaction and Optimization} (0.37) and lowest in \emph{Machine Learning} (0.22) and \emph{Applications} (0.22). This is not entirely surprising since the former two areas have a majority of reviewers from Europe, whereas the latter two have more geographic diversity. We observed a similar trend with respect to the number of papers which had coauthor reviewers. Finally, the area with maximum seniority constraint violations is \emph{Philosophy and Ethics of AI} -- probably because it is a new area and does not have many senior researchers.

%We investigated for which subject areas our matching tended to violate soft constraints. We first find a strong correlation with region violations and primary subject area. We hypothesized this was due to reviewers in these areas tending to cluster in specific geographic regions. The proportion of reviews from duplicated regions was highest in \emph{Knowledge Representation and Reasoning} (0.49) and \emph{Constraint Satisfaction and Optimization} (0.37) and lowest in \emph{Machine Learning} (0.22) and \emph{Applications} (0.22). \emph{Knowledge Representation and Reasoning} and \emph{Constraint Satisfaction and Optimization} had a majority of reviewers in Europe whereas machine learning was more evenly distributed. We observed a similar trend with respect to the number of papers which had coauthor reviewers. \emph{Knowledge Representation and Reasoning} (0.27) and \emph{Constraint Satisfaction and Optimization} had the most (0.14) and \emph{Machine Learning} (0.02) had the second fewest violations. The fewest coauthor violations came from \emph{Philosophy and Ethics of AI} (0.01). This area also stood out for violated seniority constraints, having 7.1\% of papers with no senior reviewer, % referring to seniority level 1
%near double the proportion of the next highest area (\emph{Humans and AI}). 
%Due to very few co-review violations and many seniority violations, we hypothesize that there are very few qualified reviewers for this area, so the matching has freedom to choose among most reviewers (because no one stands out) and there are no senior reviewers that match particularly well so might as well use limited highest seniority reviewers for papers that they match well with. 
%There were no clear patterns that we noticed in the few violated two-cycle violations.

\subsubsection{Was our aggscore computation stable under missing data?} 

% Two important criteria that we believe our scoring aggregation function should satisfy are (1) stability in the presence of missing data and (2) reviewers who bid positively should be rewarded if their score components are high. 
Recall that aggscore, our paper-reviewer matching score, is a combination of three constituent scores: TPMS, ACL, and SAM (see Section~\ref{subsec:scoreagg}).
%We quantified how robust our aggscore is to a missing constituent score by recomputing the aggscore in the absence of each of the constituent scores.
%For every paper, we compared the variance in the change in aggscore with the variance in the original aggscore across reviewers.
%We evaluated stability by comparing the variance in aggscores across a given paper to the variance of aggscores change when one the constituent scores is missing.
%\klb{That sentence is garbled; rephrase}
At AAAI 2021 these constituent scores were available for $60.25\%$, $96.64\%,$ and $100\%$ of papers respectively. Here we evaluate the stability of our aggscores in cases where ACL and TPMS scores were missing. 
We began with all ``qualified'' (paper, reviewer) pairs ($\scorematrixentry_{ij} \geq 0.15$) for which all of the three scores were available. 
We then computed two proxy aggregate scores, representing the scores we would have computed if either of the TPMS or ACL scores had been missing.
% The standard deviation (stdev) of the error when using the three proxy scores separately to predict the actual score, $\scorematrix$, is 
% 0.093,
% 0.033, and 
% 0.024
% respectively.

The standard deviation of the changes in aggscores caused by missing data were 0.049 and 0.048
%$0.115, 0.043,$ and $0.041$ 
respectively, whereas the mean standard deviation of the complete-data score for a given paper was 0.127.  
%For ACL and TPMS, the stdev of error is much less than the overall stdev of $0.224$ (around the mean score of $0.700$) across the matching allocated by our MIP.
Since the variance of the differences between the hidden data aggscores
and the full-data aggscores was much smaller than the average variance in aggscores across reviewers for a paper, the aggscore was still likely to have made a similar assessment of reviewer--paper pairings even in the presence of missing data.


% \subsubsection{How important were positive bids for matching?}
% \ycom{Need a discussion on this subsubsection}
% Over all matches, reviewers were assigned papers for which they bid positively (\textit{willing} or \textit{eager}) %$77.4\%$ 
% $79.2\%$ 
% of the time. A back-of-the-envelope calculation leads us to estimate that %$79.3\%$ 
% $83.0\%$ 
% of these matches
% %\klb{say XX\% of THESE matches may not have happened? That's a larger number but also easier to understand.} 
% may not have happened had the reviewer not bid positively. To calculate this, we first extracted the minimum aggscore amongst the papers' matches and considered this the lowest threshold for a match to happen on that paper, comparing to the aggscore without the reviewer's bid. This analysis ignored soft constraints, since it did not re-run the optimization to evaluate each counterfactual scenario where a bid was not submitted.
% %\nn{Is there one threshold, or is it a per-paper threshold?}.
% %\yn{per paper threshold}
% %For each match, we checked if the aggregate score before considering the reviewer bid would have still resulted in a match.

% \begin{comment}
% Stdev of the pct error when agg_score >= 0.15
% Out[53]:
% ekp    0.298562
% etp    0.195911
% eap    0.177066

% mean absolute pct error when agg_score >= 0.15
% Out[54]:
% ekp    0.780949
% etp    0.102877
% eap    0.083051
% \end{comment}

\subsubsection{How many conflicts were identified by our COI detection?}
%In this section, we analyze the additional conflicts derived from our novel extraction method of the coauthorship graph.
Let us denote self-reported conflict domains, explicitly stated conflicts, and  conflicts between coauthors of papers submitted to AAAI 2021 as `trivial conflicts'.
%Standard PRA systems rely on user-reported conflicting domains, and explicit conflicts, to identify all conflicting reviewers for a paper. In addition, we also identify a conflict between coauthors of the papers submitted to the conference. We call all such conflicts as `trivial conflicts'. 
Out of the total $2,674,372$ conflicts we found at AAAI 2021, $96.4\%$ were trivial. Of the remaining $3.6\%$ conflicts, $2.8\%$ were due to unreported coauthorship relationships we verified via DBLP. The remaining $0.8\%$ of conflicts were between predicted student--supervisor pairs or predicted students of the same supervisor. Overall, our system added at least one nontrivial conflict to a large majority ($78.8\%$) of submissions.

%% NOTE: ONLy accept/reject status papers
% Machine Learning (ML)                             0.215149
% Application Domains (APP)                         0.220109
% ....
% Constraint Satisfaction and Optimization (CSO)    0.370518
% Knowledge Representation and Reasoning (KRR)      0.487374



%%% Number of vIOLATIONS OF COAUTHOR (for any distance) divided by number of papers
% Philosophy and Ethics of AI (PEAI)                0.013514
% Machine Learning (ML)                             0.020626
% Humans and AI (HAI)                               0.024155
% Reasoning under Uncertainty (RU)                  0.028736
% Intelligent Robots (ROB)                          0.029630
% Speech & Natural Language Processing (SNLP)       0.039507
% Data Mining & Knowledge Management (DMKM)         0.044776
% !Focus Area                                       0.047198
% Application Domains (APP)                         0.048007
% Human-Computation and Crowd Sourcing (HCC)        0.054545
% Search and Optimization (SO)                      0.075117
% Computer Vision (CV)                              0.075453
% Multiagent Systems (MAS)                          0.113821
% Game Theory and Economic Paradigms (GTEP)         0.126565
% Planning, Routing, and Scheduling (PRS)           0.137931
% Constraint Satisfaction and Optimization (CSO)    0.143426
% Knowledge Representation and Reasoning (KRR)      0.265152
% Cognitive Modeling & Cognitive Systems (CMS)           NaN




% Looking at number of papers with no seniority level 1 reviewer by number of papers in that subject area
% !Focus Area                                       0.000000
% Reasoning under Uncertainty (RU)                  0.000000
% Planning, Routing, and Scheduling (PRS)           0.000000
% Knowledge Representation and Reasoning (KRR)      0.000000
% Intelligent Robots (ROB)                          0.000000
% Human-Computation and Crowd Sourcing (HCC)        0.000000
% Multiagent Systems (MAS)                          0.016667
% Speech & Natural Language Processing (SNLP)       0.017350
% Search and Optimization (SO)                      0.018519
% Game Theory and Economic Paradigms (GTEP)         0.021622
% Cognitive Modeling & Cognitive Systems (CMS)      0.024390
% Application Domains (APP)                         0.024823
% Machine Learning (ML)                             0.025116
% Computer Vision (CV)                              0.026349
% Data Mining & Knowledge Management (DMKM)         0.031250
% Constraint Satisfaction and Optimization (CSO)    0.032258
% Humans and AI (HAI)                               0.038462
% Philosophy and Ethics of AI (PEAI)                0.071429





==> aaai21_paper_reviewer_matching (5)/two_phase.tex <==
% \cc{never say here that we actually did this at AAAI 2021.}
% \nn{Need to say that other conferences have followed us and are also using 2-phase reviewing. At least the next year's AAAI}
% \hz{I think these would work better if added to the into}
The quality of papers submitted to large conferences such as AAAI 2021 varies vastly. An influential experiment by organizers of the 2014 NeurIPS conference \citep{lawrence&al17} split reviewing between two independent Program Committees and had them both review 10\% of submissions. It found that the strongest papers (a small set) and the weakest papers (a much larger set) could be reliably identified, but that many papers close to the decision boundary were accepted by one Program Committee and rejected by the other. In the years since, conference organizers have sought to reallocate reviewing resources from papers that are nearly certain to be rejected to papers that have a realistic chance of acceptance, to improve review quality for the latter group. A popular approach is to employ simple heuristics designed to detect low-quality papers, a process known as ``summary rejection'' or ``desk rejection''.
For example, in IJCAI 2020, Area Chairs were asked to spend a short amount of time skimming each paper to decide whether it deserved a more careful review \citep{bessiere&al20}.
Neurips 2020 employed a similar system: over three weeks, Area Chairs skimmed over 9,000 papers to identify obvious rejects and senior Area Chairs cross-checked these choices; 11\% of submissions received summary rejects \cite{yuan&al20}. Given the size of AI conferences, such summary rejection procedures are time consuming for Area Chairs. Furthermore, they are likely to be noisy and also may reflect unconscious biases against superficial properties of a paper, meaning that they may not be reliable enough to eliminate more than a relatively small fraction of papers. Finally, they tend to be unpopular with authors, who dislike having their paper rejected via an opaque process that produces no reviews. For these reasons, NeurIPS decided not to employ such an approach in 2021 on the basis of negative feedback received in 2020.

We advocate an alternative early-rejection approach that simultaneously concentrates the conference's reviewing budget on papers close to the decision boundary; provides meaningful feedback to authors of early-rejected papers; and early-rejects few papers that could ultimately have been accepted (see our evaluation below). The key idea is to break reviewing into two phases. {In Phase 1} each paper is assigned 2 reviewers. Papers that receive two sufficiently-high-confidence reviews recommending rejection are rejected at this stage, with the authors immediately receiving these full reviews and being offered no opportunity for rebuttal. The process then proceeds to Phase 2, where two or more additional reviewers are assigned to each of the papers that remain. After the second round of reviews, rebuttals are solicited from authors and reviewers from both phases are asked to read rebuttals and each other's reviews, to engage in a discussion mediated by SPCs and ACs, and ultimately to revise their reviews accordingly. Program Chairs then make decisions based on recommendations from ACs.

The key rationale for this system is that, given the low acceptance rates at AI conferences, papers for which the first two reviews are both confident and negative have a very low chance of eventual acceptance. Because reviews are much more careful than quick perusals by ACs, this system is also able to reject a larger fraction of papers than the summary rejection approaches employed by IJCAI, NeurIPS, and other conferences. The resulting reviewing resources can be devoted to papers with a larger chance of acceptance, reducing variance in these recommendations. In the experimental section below, we offer evidence both that papers rejected in Phase 1 were indeed likely to be rejected if given more reviews, and that additional reviews performed in Phase 2 indeed reduced variance in confidence-weighted average scores. 

It is also worth mentioning three additional benefits of the Two-Phase approach. First, inevitably some reviewers fail to complete their assignments, others report low confidence, and still others point out a need for additional reviews by specialists in particular topics. When this occurs in Phase 1, new reviewers can be found without needing to resort to ad hoc, manual approaches that scale badly to large conferences. 
Second, the existence of a second reviewer--paper matching period at the beginning of Phase 2 makes it possible to fast-track high-quality rejected submissions from another conference, using their previous reviews and some numerical constraint on their average scores to take the place of the reviews that would have been obtained in Phase 1. We deployed such a ``fast-track'' in AAAI 2021 for papers that received NeurIPS and EMNLP reviews that scored them roughly in the top half of submissions. Third, many authors appreciate receiving rejection notifications quickly so that they can resubmit their work to another venue without waiting for the whole review process to conclude.

Finally, we note two key drawbacks of Two-Phase reviewing: reviewers have to be chased twice, increasing workload for Program Chairs, ACs, and SPCs; and authors rejected in Phase 1 have no opportunity to rebut reviews that they consider erroneous.


While we designed our Two-Phase reviewing system independently, we have since learned that various versions of the idea were previously implemented at several other CS conferences. To the best of our knowledge, the first conference that split reviewing into two phases was ICML 2009~\cite{Bottou}. According to the program chairs, the motivation was not increasing the number of reviews assigned to strong papers, as it was for us, but rather a concern that papers would be rejected by reviewers who did not fully understand them, due to exponential growth in submissions that had led to a pool of papers larger than the pool of trusted reviewers. ICML09’s system differed from ours in at least two key ways: in Phase 1, authors in ICML 2009 were asked to indicate a preference for an Area Chair who would oversee their paper in Phase 2 and help to choose reviewers; papers were allowed to submit a rebuttal in response to Phase 1 reviews. Two-Phase reviewing was discontinued at ICML in 2011, apparently because the highly manual process became both logistically unwieldy and excessively time consuming as the conference continued to grow.


%{\color{red}While we designed our Two-Phase reviewing system independently, we have since learned that various similar systems were previously implemented at several other CS conferences. To the best of our knowledge, the first conference that split reviewing into two phases was ICML 2009~\cite{Bottou}.  
%\cc{I don't understand this sentence below. They switched to two phase because unqualified rejections? Is this unqualified desk rejections? Should say if so. Not obvious why two-stage would fix unless it is was specifically about desk rejects}
%\yn{Does it make sense if you read it with the first key difference? The source of this info is the email from ICML09 chairs... So instead of saying `Key differences from ..', should we say: 'Hence, authors in ICML09 were asked ..' }
%According to the program chairs, the motivation was not increasing the number of reviews assigned to strong papers, as it was for us, but rather a concern that papers would be rejected by reviewers who did not fully understand them, due to recent, exponential growth in submissions that had led to a pool of papers larger than the pool of trusted reviewers. ICML09's system differed from ours in at least two key ways: in Phase 1, authors in ICML 2009 were asked to indicate a preference for an Area Chair who would oversee their paper in Phase 2 and help to choose reviewers;
%\nn{I have no idea what it means for an AC to handle my paper}\cc{I assume means pick AC to "review" paper?}\yn{Yes, I have changed the text to reflect this}\klb{I'm sure it meant the same thing as assigning an AC for us. Not another review.}
%papers were allowed to submit a rebuttal in response to Phase 1 reviews. Two-Phase reviewing was discontinued at ICML in 2011, apparently because the highly manual process became both logistically unwieldy and excessively time consuming as the conference continued to grow.
%\st{the Two-Phase process left very little time for author responses and discussion due to the increasing size of the conference}
%\nn{Again, shouldn't we have the same problem at AAAI if this were the case? If not, what exactly did we do differently that made it work? I'd rather not give a reason at all and just say it was abandoned than say this}\yn{Please see if this makes more sense}

We are aware of two other (non-AI) conferences that also employed Two-Phase reviewing: ASPLOS, and OOPSLA \cite{Adve2010,10.1145/2641638.2641648}. Notably, in OOPSLA13~\cite{10.1145/2641638.2641648}, authors of accepted Phase 1 papers were asked to revise their papers based on Phase 1 reviews; Phase 2 reviews then assessed the revised versions. 
%We consider the emergence of Two-Phase reviewing across diverse communities and with subtly different implementations as an endorsement of its efficacy. 
ASPLOS21~\cite{Kozyrakis2021} required authors to submit a two-page extended abstract in Phase 1; about 55\% of the papers were then promoted to Phase 2 and asked to submit a full paper. In addition to these conferences, \citet{Hans} describe a Two-Phase reviewing process for PLDI conferences, in which Phase 1 decisions are made based on at least three reviews and authors of the papers that are candidates for Phase 1 rejection are invited to submit author responses before a final decision is made for their papers. The author response period for the rest of the papers happens at the end of Phase 2.

AAAI 2021's successful deployment of Two-Phase reviewing has already begun to show some impact of its own. On the practical side, our Two-Phase design was maintained by AAAI 2022 and was newly adopted by both IJCAI 2022 and ICML 2022. The design has also received academic study. A recent paper by \citet{https://doi.org/10.48550/arxiv.2108.06371} investigated how reviewers should be divided across the two phases to maximize the overall matching score in a conference, showing that the problem is NP-Hard and empirically verifying that a simplified \textit{random-split} strategy of randomly reserving reviewers for Phase 2 gives a near-optimal assignment on real conference data.



==> aaai21_paper_reviewer_matching (5)/two_phase_evals.tex <==
%In this section, we evaluate our two-phase design in four different ways, using data gathered from our conference.

\subsubsection{How prevalent were false negatives?}\label{sec:false-negatives} 
The risk we were most concerned about arising from our Two-Phase design was the possibility that papers rejected in Phase 1 might have been accepted if they had received additional reviews, an opportunity for rebuttal, and/or discussion; we call such papers ``false negatives''. The cleanest way to estimate the probability with which we falsely rejected such papers in Phase 1 would have been for us to conduct a randomized experiment: randomly promoting some fraction of papers that would otherwise have been rejected in Phase 1 and observing the result. We did not perform this experiment, but the real data provides a very similar natural experiment. Specifically, we promoted papers to Phase 2 without considering their scores in two cases: (1) when one or more reviews were missing; and (2) when their reviewers had low confidence. In total, 231 papers were promoted in this manner, 16 of which were eventually accepted. Each of these papers eventually received four or more high-confidence reviews, allowing us to calculate the probability that two randomly selected reviews would have met the criteria for Phase 1 rejection. This allowed us to estimate what fraction of Phase 1 rejections might eventually have been accepted. In our data this probability was  $2.9\%$, suggesting that Phase 1 rejections included very few false negatives.

%126 papers were promoted as one or more reviews were missing and finally 8 out of these 126 were accepted.
%105 papers were promoted because of low confident reviews. 8 out of these 105 were accepted.

\subsubsection{Did Phase 1 reviewers participate in discussion after Phase 2?} There was a relatively long delay between the end of Phase 1 and the start of the discussion period (in our case, almost a month), leading to some public speculation that Phase 1 reviewers might have tended to be less active in the discussion phase~\cite[e.g.,][]{Kambhampati}. We found little evidence of such a trend: Phase 2 papers received a discussion post from 55\% of Phase 1 reviewers and likewise 55\% of Phase 2 reviewers. We did find that reviewers who reviewed only in Phase 1 (who were responsible for a relatively small fraction of reviews overall) had a slightly smaller (52\%) rate of participation in the discussion. We further note that Two-Phase reviewing is not the only possible explanation for this small discrepancy: e.g., this group may also have contained a smaller fraction of highly qualified reviewers.

% 2400 FT Reviews
% 22329 Main Track
% 450 AISI

% 711 papers recieved more than 4 reviews
%  769 papers in fast track received any reviews

%\subsubsection{Were Phase 2 reviewers more likely to change their scores after rebuttal?}

% 1. Prob of changing score | phase
% 2. Negative/positivity bias in score change | phase


\subsubsection{How many additional reviews were gained?} AAAI 2021 received 7,133 full paper submissions to the first phase. %The total number of reviews submitted by reviewers across both phases was {25,179}. \yn{this means that we anyway had the capacity to get 4 reviews per paper(6192*4 = 24768)} To assign every Phase 1 paper three reviews would have required {20,631} reviews. \yn{Why is this statement relevant for the calculations below?} 
We were able to reject 2,615 (about $37\%$) of the submitted papers in Phase 1, leaving us with a surplus of {2,615} reviews (relative to AAAI's previous practice of assigning 3 reviews to each paper) to spread amongst the remaining papers. %In Phase 2, 769 fast track submissions required reviewing.
 This contributed towards assigning
 at least four reviewers to every main track paper in Phase 2 and at least 3 reviews to the 737 fast track submissions, out of which 721 submissions received more than 4 reviews.%\yn{4 reviewers in total, or 4 reviewers only in phase 2?}
%\yn{In this discussion, we are not accounting for additional reviews required for the fast track submissions. That increased the total number of required reviews, and it wouldn't have been possible to accomodate them without the additional capacity gained due to phase 1 rejects.}
    
\subsubsection{How important was it to have additional reviews?} 
%\ycom{Need discussion on this subsubsection}
For every Phase 2 paper, we sampled every subset of 3 reviews that it might have received if a subset of the same reviewers had been assigned in a single-phase conference and calculated the confidence-weighted average score that the paper would have received in this scenario. (Confidence ranged between 1 (low) and 4 (high); corresponding weights were 0.25, 0.5, 0.75, and 1.) 
% NN - We could not verify this in any CMT docs or find it on our interface so do not want to claim this
%We chose these values to follow the formula used in CMT, which is a key quantitative metric presented in the SPC, AC and Program Chair user interfaces.) 
We plot the result in Figure~\ref{fig:aaai_score_variance}. Each point corresponds to a 3-review scenario for a single paper. The $x$ axis gives the paper's score in the AAAI 2021 conference (where it received more than 3 reviews); the $y$ axis gives the spectrum of 3-review scores. The decision boundary for acceptance fell around 6.4, though many papers below this threshold were accepted and many above this threshold were rejected. Nevertheless, variance in the score is a good proxy for variance in reviewer support for the paper. Figure~\ref{fig:aaai_score_variance} shows that for papers that are close to the decision boundary, the weighted average score could vary by up to 2 points around the threshold depending on which 3-reviewers were picked, implying that decisions for these papers could be very uncertain with only 3 reviewers. Therefore, we conclude that the additional reviews enabled by two-phase reviewing helped Program Chairs to make more confident decisions, specially about papers that are close to the decision boundary. 
% and increasing the number of reviews for a paper can only  decrease the variance in the estimate of its true score.
%\st{increase this variance.} \todo{Yatin: please check.}
%Overall, we conclude that the additional reviews enabled by two-phase reviewing substantially reduced variance in paper scores, particularly for papers close to the decision boundary.
%\yn{In this graph, we are showing the variance in the estimate of mean review score when mean is estimated using 3 samples. How does it show that variance in the mean estimated in AAA21 is substantially reduced?}
%\yn{Instead, should we plot the computed variance vs number of reviewers assigned (instead of conference score), and show that when variance for a paper was high, we indeed ended up assigning more reviewers to it, and it was possible due to 2 phase reviewing?}

% Papers by status
%Reject                    0.327294
%Phase 1 Reject            0.265926
%Accept                    0.193337
%Withdrawn                 0.134658
%Desk Reject               0.071537
%Dual Submission Reject    0.007247
% Reject
% Lean reject
% Lean accept
% Weak accept
% Accept
% Best paper
% Total

\begin{figure*}
    \centering
  \includegraphics[width=.6\textwidth]{figures/score_variance_3}
  \caption{Confidence-weighted average scores for Phase 2 papers based on all reviews vs.\ all combinations of 3 reviews. Marginal densities are plotted on the sidelines. \label{fig:aaai_score_variance}}
\end{figure*}

\subsubsection{Did the adoption of Two-Phase reviewing result in a higher bar for acceptance by ACs/SPCs?}
%\nn{This question isn't "natural" to ask IMO. Maybe cite the tweet that prompted it?}
One concern that has been publicly raised about two-phase reviewing is that it might depress acceptance rates because ACs and SPCs may aim to accept the same fraction of Phase 2 papers as in previous years, not considering the large fraction of papers already rejected in Phase 1  \cite[e.g.,][]{Walsh2022}. Our analysis of AC/SPC recommendations shows that this was not the case in AAAI 2021. ACs submitted 3,825 ratings on a scale of \textit{Reject, Lean Reject, Lean Accept, Weak Accept, Accept, and Best Paper}. Considering the last four scores as recommendations for acceptance, we found that ACs recommended accepting $37.6\%$ of Phase 2 papers, corresponding to an overall acceptance rate of $22.2\%$. Similarly, SPCs submitted 3,873 ratings on a scale from 1 to 9.\footnote{The text prompts given for each score were as follows: (1) Trivial, wrong, or known; (2) Strong reject: will fight to get it rejected; (3) Clear reject; (4) Reject; (5) Below threshold of acceptance; (6) Above threshold of acceptance; (7) Accept; (8) Clear Accept (Top 50\% accepted papers (est.)); and (9) Accept: will fight to get it accepted.} Considering scores above 5 as accept recommendations, SPCs recommended accepting $37.5\%$ of Phase 2 papers, corresponding to an overall acceptance rate of $22.3\%$.
%Tables~\ref{tab:ac_ratings} and~\ref{tab:spc_ratings} summarize AC and SPC ratings respectively and demonstrate that if Program Chairs had followed the recommendations exactly, the acceptance rate of AAAI 2021 would have been about $22\%$ 
Both of these percentages were higher than the conference's actual acceptance rate of $21\%$ and almost the same as the average acceptance rate of $22.9\%$ over the last 5 years~\cite{openresearch}. We therefore see no evidence to support the claim that introducing two-phase reviewing leads to lower overall acceptance rates.



%This means that Program Chairs have decided to overrule some of the ACs/SPCs ratings.   
%\nn{I think both tables are unnececessary - I'm not sure what I gain by having access to so many numbers. I would just say }
%\cc{I agree}
%\nn{Is there a danger here that we are ignoring the fact that some papers might be rejected independently by ACs OR SPCs but not both? Maybe when you look at the union, the acceptance ratio would be lower}
%\hz{This might be actually true, but I think we dont need to take that into account. Here we are just answering a slightly different question I think}
% \begin{table*}
% \begin{center}
% \small
% \begin{tabular}{ l| r r r r}
% \toprule
%  \textbf{AC rating} & \textbf{Count} & \textbf{Fraction} & \textbf{Cumulative} & \textbf{Acceptance ratio if rejected until rating}\\
%  \midrule
%     Reject	& 1629	& 0.426	& 0.426	& 0.340 \\
%     \textbf{Lean reject}	& \textbf{759}	& \textbf{0.198}	& \textbf{0.624}	& \textbf{0.222} \\
%     Lean accept	& 303	& 0.079	& 0.704	& 0.175 \\
%     Weak accept	& 421	& 0.110	& 0.814	& 0.110 \\
%     Accept	& 701	& 0.183	& 0.997	& 0.002 \\
%     Best paper	& 12	& 0.003	& 1.000	& 0.000 \\
%  %' Match Quality & 40.9 & ?\\
%   \bottomrule
% \end{tabular}
% \caption{Statistics of paper count by AC rating. The acceptance ratio column takes into account the papers rejected in Phase 1.}
% \label{tab:ac_ratings}
% \end{center}
% \end{table*}

% \begin{table*}
% \begin{center}
% \small
% \begin{tabular}{ l| r r r r}
% \toprule
%  \textbf{SPC rating} & \textbf{Count} & \textbf{Fraction} & \textbf{Cumulative} &
%  \begin{tabular}[c]{@{}r@{}}\textbf{Acceptance ratio} \\ \textbf{(if rejected until rating)}\end{tabular} \\ \midrule
%     Trivial, wrong, or known 	& 4	& 0.001	& 0.001	& 0.594 \\
%     Strong reject & 22	& 0.006	& 0.007	& 0.591 \\
%     Clear reject	& 214	& 0.055	& 0.062	& 0.558 \\
%     Reject & 1113	& 0.287	& 0.349	& 0.387 \\
%   \textbf{Below threshold of acceptance}	& \textbf{1067}	& \textbf{0.275}	& \textbf{0.625}	& \textbf{0.223} \\
%     Above threshold of acceptance	& 729	& 0.188	& 0.813	& 0.111 \\
%     Accept	& 578	& 0.149	& 0.962	& 0.022 \\
%     Clear Accept & 129	& 0.033	& 0.996	& 0.003 \\
%     Accept: will fight to get it accepted	& 17	& 0.004	& 1.000	& 0.000 \\
%  %' Match Quality & 40.9 & ?\\
%   \bottomrule
% \end{tabular}
% \caption{Statistics of paper count by SPC rating. The acceptance ratio column takes into account the papers rejected in Phase 1.}
% \label{tab:spc_ratings}
% \end{center}
% \end{table*}

\subsubsection{Did reviewers behave differently in Phase 2?}
%- data analysis shows that reviews are more negative in phase 2 on the same set of papers
%    - the difference is more significant on borderline papers
%    - support by statistical tests
In AAAI 2021, Phase 2 reviews tended to be (slightly) more negative than Phase 1 reviews, with Phase 1 pre-rebuttal scores averaging 0.29 higher than Phase 2 pre-rebuttal scores on the 10-point scale (see Figure~\ref{fig:ecdf} for an ECDF).  We used the Wilcoxon signed-rank test \cite{Rey&neuh11} to check whether pairs of Phase 1 and Phase 2 reviews given to the same paper came  from the same distribution (null hypothesis) or whether Phase 2 reviews tended to be more negative (alternative hypothesis). We ran the test with a significance level of 0.01 on a dataset whose entries were every possible combination of a Phase 1 review score and a Phase 2 review score for the same paper. (Thus, we only considered papers which were reviewed in Phase 2.)
%We performed a statistical test to see whether the difference between Phase 1 and Phase 2 reviews is statistically significant or not. 
We used pre-rebuttal scores %\nn{Didn't we have ambitions to add another question to this section about rebuttal scores?} 
to make sure that reviewers' scores were not influenced by reading author responses and other reviews, after which review scores tended to become more correlated). 
%\nn{How big is the dataset in terms of pairs, not just in terms of papers}
Over 6160 pairs of scores in our dataset%\nn{IIRC, whether you have a pre-rebuttal score or not is a function of the reviewer, and not the paper. I think some sort of data cleaning comment is needed here to say that we simply weren't always able to get access to the pre-rebuttal score}
, the test had a $p$-value of $7.57 \times e^{-69}$, causing us to reject the null hypothesis that reviewing was identical across phases. %\cc{Think we needed to have picked a significance level a priori. I took a shot at changing the text. Not sure the correct format for presenting the test}

\begin{figure*}
    \centering
    \includegraphics[width=.6\textwidth]{figures/ecdf.pdf}
    \caption{ECDF of the review scores by review phase. Phase 2 reviews tend to be more negative than Phase 1 reviews.\label{fig:ecdf}}
\end{figure*}



There are various reasons why reviewers might have been more negative in Phase 2: they may have applied a higher standard, knowing this was the final reviewing round; they may have changed their perceptions about quality thresholds after their experiences reviewing in Phase 1; more qualified reviewers might have been identified in Phase 2 and these reviewers may have had more critical views. 

However, a fourth explanation occurred to us, which the data can tell us something about: reviewers may have behaved exactly as they did in Phase 1, but the change in scores might have arisen due to selection bias arising from the Two-Phase structure. %: noisy review scores allow some fraction of ``bad'' papers to erroneously slip through to Phase 2. This is not a symmetric effect, as ``good'' papers erroneously marked as ``bad'' are removed from the conference. To make this hypothesis concrete, 
To see how this might have happened, imagine that each reviewer's score is an unbiased sample from a Gaussian centered on the ``true score'' of the paper. %Then a reviewer's score will half of the time be a bit higher than the true score of the paper and half of the time be a bit lower. Papers with low true scores that receive two low reviews in Phase 1, do not participate in this study as they do not receive any Phase 2 scores.
While reviewing in this model is unbiased on expectation, performing reviewing in two phases adds bias. That is, if both reviewers in Phase 1 draw samples above the paper's true score, the paper will get more reviews in Phase 2, which on expectation will be more negative. Conversely, if both reviewers in Phase 1 draw samples well below the paper's true score, we'd again expect additional reviews to revert to the mean, but we will not see those additional reviews because the paper will be rejected in Phase 1. This asymmetry means that we should expect reviews in the second phase to be more negative on average for purely statistical reasons; observing such bias is not necessarily cause for alarm.

To investigate the impact of this selection bias effect, we considered a refined dataset of papers that had at most 1 negative review (review score of 5 or below), and hence would not have been rejected in Phase 1 regardless of the order in which their reviewers were chosen; there turned out to be 1583 papers. We again ran the Wilcoxon signed-rank test comparing Phase 1 scores to Phase 2 scores and obtained a $p$-value of $0.57$: we did not have enough evidence to reject the null hypothesis that the distributions of Phase 1 scores and Phase 2 scores were the same. This indicates that these papers were unlikely to have been promoted from Phase 1 purely due to noise.

We now turn to a more quantitative analysis. To see how much of the 0.29-point average score gap between reviews in the two phases could plausibly be explained by selection bias, we needed to estimate the variability of reviewers' process of scoring papers. We thus constructed a simple statistical model of our setting. We assumed that each paper $p$ has a true score $s_p \in \mathbb{R} $ which is drawn from a Gaussian distribution $\mathcal{N}(\mu_s, \sigma^2_s)$ where $\mu_s$ and $\sigma^2_s$ indicate our prior belief on the average and variance of true scores. 
%\yn{But aren't review scores sampled from a discrete distribution (10,9,8...)? Do we want to talk about the mean of this distribution here?}
When asked to review paper $p$, reviewer $r$ draws an unbiased sample $o^p_r$ from a normal distribution $\mathcal{N}(s_{p}, \sigma^2)$ around $s_p$, the true score of paper $p$, and with the variance of $\sigma^2$. We note that when we use thousands of observations to fit a handful of parameters, priors are overwhelmed and hyperparameter choices become nearly irrelevant. Nevertheless, performing Bayesian inference requires the selection of priors. We therefore estimated $\mu_s=5$ and $\sigma^2_s=1$ as the empirical mean and variance of overall paper scores and assumed that the prior over $\frac{1}{\sigma}$ was $\GammaDist(\alpha_\tau, \beta_\tau)$, setting $\alpha_\tau= \beta_\tau = 1$.
% Formally:

% \begin{align*}
%     \text{(True scores)}& \quad 
%     s_{p} \sim \mathcal{N}(\mu_s, \sigma_s^2); \\
%     \text{(Reliabilities)}& \quad 
%     \frac{1}{\sigma} \sim \GammaDist(\alpha_\tau, \beta_\tau); \\
%     \text{(Observed scores)}& \quad
%     o_{p}^r \sim \mathcal{N}(s_{p}, \sigma^2).
% \end{align*}
% , where $\tau = \frac{1}{\text{reviewers' variance}^2}$.
% \yn{Then shouldn't $\quad
%     o_{p}^r \sim \mathcal{N}(s_{p}, 1/\tau)$}
%We assume that reviewer $r$ maps her observation $o^p_r$ to a discrete report $d^p_r \in \{1,\dots,10\}$. 
We used Gibbs sampling to estimate $\sigma$ for reviewers and $s_p$ for every $p$. After taking the average over the Gibbs samples, our inference estimated $\sigma$ to be $1.3$.
%\yn{I think we need to estimate other parameters as well for our similation. Let's metion their value as well?}
We then ran a simulation in which we used our graphical model to generate 6,723 true paper scores\footnote{6,723 is the total number of papers in our database that were either rejected or accepted based on their reviews in Phase 1 or Phase 2---i.e., excluding papers that left the system for other reasons, such as being withdrawn by their authors or being desk rejected because of double submission, violation of author anonymity, exceeding page limits, etc.} from $\mathcal{N}(5, 1)$ and review scores that followed the noise model defined by $o_{p}^r \sim \mathcal{N}(s_{p}, 1.3^2)$. 
%\yn{But the observed scores are $d_r^p$ and not $o_r^p$? Are we generating 3788 samples in the simulation? Or are we saying that we used the 3788 samples that we had to estimate the parameters?}
We then simulated Phase 2 by filtering out any paper that received two reject recommendations (received two review scores below 4.5) from its first two sampled review scores (in Phase 1). Considering the remaining (Phase 2) papers in our synthetic experiment, we observed that Phase 1 reviews were $0.18$ higher than Phase 2 reviews on average. Overall, this (simplistic) analysis explains about two thirds of the gap that we saw in our real data. We conclude that selection bias likely made reviewing in the two phases appear more different than it really was, but that it is furthermore plausible that reviewers did behave at least somewhat differently in the two phases. 

%We ran a small experiment to figure how big reviewers' variance should be for to see the gap that we saw between Phase 1 and Phase 2 average review scores. We first 
% inference to figure the variance of reviewers. 
% - we run a small inference to figure the variance of reviewers
% - with this variance we run a simulation that shows this can explain about half of the gap
% - this only explains about half of the gap

    
% 1. Significantly more negative reviews in phase 2.
% 2. Is there a correlation between negativity bias and paper score. If not, does the falsify the theory of negativity bias via filtering bad papers? How strong should we expect the correlation to be in that case. 



